Preference-Based Planning in Stochastic Environments: From Partially-Ordered Temporal Goals to Most Preferred Policies

Human preferences are not always represented via complete linear orders: It is natural to employ partially-ordered preferences for expressing incomparable outcomes. In this work, we consider decision-making and probabilistic planning in stochastic systems modeled as Markov decision processes (MDPs), given a partially ordered preference over a set of temporally extended goals. Specifically, each temporally extended goal is expressed using a formula in Linear Temporal Logic on Finite Traces (LTL$_f$). To plan with the partially ordered preference, we introduce order theory to map a preference over temporal goals to a preference over policies for the MDP. Accordingly, a most preferred policy under a stochastic ordering induces a stochastic nondominated probability distribution over the finite paths in the MDP. To synthesize a most preferred policy, our technical approach includes two key steps. In the first step, we develop a procedure to transform a partially ordered preference over temporal goals into a computational model, called preference automaton, which is a semi-automaton with a partial order over acceptance conditions. In the second step, we prove that finding a most preferred policy is equivalent to computing a Pareto-optimal policy in a multi-objective MDP that is constructed from the original MDP, the preference automaton, and the chosen stochastic ordering relation. Throughout the paper, we employ running examples to illustrate the proposed preference specification and solution approaches. We demonstrate the efficacy of our algorithm using these examples, providing detailed analysis, and then discuss several potential future directions.

==> archieved/deciding_if_proper_policy_exists.tex <==
 \subsection{Deciding If the Problem Has a Solution}
    %
    After constructing the product MDP, the algorithm checks whether there exists a proper policy for $M$ or not.
	%
	If not, then the algorithms returns `\textsc{NoProperPolicyExists}', otherwise, it compute the set of weak-stochastic nondominated policies as it was dissucced in the previous section. 
	%
	There exists a proper policy for $M$ only if the $\calM$ has no unavoidable \emph{dead end}---a state from which no goal state is reachable. 
	%
	Consider Figure~\ref{fig:deadends} and
	read~\cite{bertsekas1991analysis, kolobov2012theory, little2007probabilistic, kolobov2010sixthsense, keyder2008hmdpp, bonet2003faster} for more detail about proper polices and dead-ends\gobble{, including algorithms to detect dead-ends and strategies to handle them}.
% 	To illustrate consider Figure~\ref{fig:deadends}, which shows two product MDPs.
% 	%
% 	In each MDP, state $x_3$ is a dead end. That state in the MDP shown in part a) of the figure is avoidable, by not allowing action $b$ to be chosen at state $x_0$ and by not allowing action $a$ to be chosen in state $x_2$.
% 	%
% 	Accordingly, there exists at least a proper policy for that MDP.
% 	%
% 	In contrast, state $x_3$ in the MDP shown in part b of the figure is unavoidable, and hence, there is no proper policy for that MDP.
	%
	
	\begin{figure}[h]
		\centering
		\includegraphics[width=1.0\linewidth]{figures/DeadEnds.pdf}
		\caption{
		 \textbf{a)} An MDP with an avoidable dead end. State $x_3$ is a dead end, but it is avoidable (by not allowing actions $b$ and $a$ to be chosen respectively at states $x_0$ and $x_2$). In this case, a proper policy for the product MDP exists.
		 \textbf{b)} An MDP with an unavoidable dead end, $x_3$. In this case, there is no proper policy for 
		 the product MDP.
		}
		\label{fig:deadends}
	\end{figure}
% 	\jf{the discussion of dead end seems to dilute the main message. can you check the stochastic shortest path literature where proper policies are also introduced and cite these? check out \url{https://www.mit.edu/~dimitrib/Stochasticsp.pdf} the assumption 1. we only need to enforce such an assumption and add that all improper policies will receive a reward of zero. the contraction property can be maintained. }
	
% 	\hrm{
% 	  Sure, we need to cite papers, but probably if we can allocate a minimum space, perhaps only the picture, it would be good for the reader.
% 	}

==> archieved/sections/intro.tex <==
% What are incomplete preferences? 
% Why should roboticists care about incomplete preferences over finite words? 
% What are conventional assumptions in standard decision theory?
% What are its limitations? 
% How do we address these limitations? Why do we choose automata theoretic approach? 
% What will be the impact of our work? 


Preference-based planning decides what constraints to satisfy when not all constraints can be achieved \cite{hastie2010rational}. In this paper, we study a class of qualitative, preference-based probabilistic planning problem in which the agent aims to strategically exploit the \emph{opportunities} that arise due to stochasticity in its environment to achieve a more preferred outcome than what may be achieved from its initial state. Such problems are encountered in many applications of autonomous systems.    


In existing methods for probabilistic planning with temporal goals, the desired behavior of the system is specified by a temporal logic formula \cite{manna2012temporal}, and the goal is to compute a policy that either maximizes the probability of satisfying the formula \cite{ding2011mdp,hasanbeig2019reinforcement}, or enforces the satisfaction as a constraint  \cite{Lacerda2014,wen2015correct}. In recent work, preference-based planning with temporal logic objectives have been studied: minimum violation planning in a deterministic system \cite{tumova2013least} decides which low-priority constraints to be violated. Automated specification-revision is proposed in \cite{Lahijanian2016} where the formula can be revised with a cost and the planning problem is formulated into a multi-objective \ac{mdp} that trades off minimizing the cost of revision and maximizing the probability of satisfying the revised formula. \cite{mehdipourSpecifyingUserPreferences2021} introduced weights  with Boolean and temporal operators in signal temporal logic to specify the importance of satisfying the subformula and priority in the timing of satisfaction. They developed a gradient-based optimization method to maximize the weighted satisfaction in deterministic dynamical systems. Robust and recovery specifications are introduced by \cite{bloem2019synthesizing} and pre-specify what behaviors are expected when the part of the system specification (\ie,  the environment assumption) fails to be satisfied. Existing  preference-based planning methods with temporal goals assume the preference relation to be \emph{complete}.  

Unfortunately, in many  applications, the completeness assumption does not always hold. For instance, it can be impractical to elicit user's preference between every pair of outcomes when the set of outcomes is large; or in some situation, such as the trolley problem \cite{thomson1976killing}, the outcomes (sacrificing passengers or pedestrians) are incomparable. Preference languages have been proposed to represent both the complete and incomplete preferences over propositional formulas  \cite{van2005preference} and temporal logic formulas \cite{bienvenuPreferenceLogicsPreference2010}. For planning, CP-net and its variants \cite{santhanam2016representing,boutilier2004cp} have been proposed as a computational model. But they are defined over propositional preferences. To the best of our knowledge, there is no computational model that can express incomplete preferences over temporal goals. Such a model is needed to facilitate planning in stochastic environments. 

In this paper we make several contributions: (1) in Section~\ref{sec:def}, we propose to use a finite automaton, we call preference deterministic finite automaton, to specify user preferences over time-extended goals where the relation between the preferences is a partial order rather than a total order (2) in Section~\ref{sec:def}, we present a problem formulation for preference-based temporal planning in stochastic environments, modeled as an MDP, using the notion of weak-stochasticity for ranking different policies, and (3) in Section~\ref{sec:alg}, we propose our algorithm to solve the problem.
%
Our algorithm reduces the problem of computing the set of weak-stochastic nondominated polices for the input MDP of the problem into the problem
of computing the set of nondomianted polices for a product MDP it makes from the inputs of the problem.

==> figures/ex-pdfa-pgraph.tex <==

\begin{tikzpicture}[ ->, node distance=2cm,    el/.style = {inner sep=2pt, align=left, sloped},
	scale = 1,transform shape]
	
	\node[state] (2) {$\{2\}$};
	\node[state] (3) [right of=2] {$\{3\}$};
		\node[state] (1) [above  of=3] {$\{1\}$};
	\node[state] (4) [ right of=3] {$\{4\}$};
	
	\path (2) edge                  (1)
	(3) edge                  (1)
	(4) edge                  (1) ;
	
\end{tikzpicture}

==> sections/case_study.tex <==
In this section, we present the results from the planning algorithm for the running example in Figure~\ref{fig:gap_garden}. 
We implemented this case study in Python. 
All the experiments were performed on a Windows 11 installed on a device with a core i$9$, 2.50GHz CPU and a 32GB memory. 


%
In the garden, the actions \replaced{available to}{of} the robot are $N$, $S$, $E$, $W$--- corresponding to moving to the cell in the North, South, East, and West side of the current cell, respectively---and $T$ for staying in the current cell. The bee robot initially has a full charge, and using that charge it can fly only $12$ time steps.
%\aknote{Didn't understand what is meant by receptively?}

\noindent \textbf{Uncertain environment. } A bird roams about  the south east part of the garden, colored yellow in the \replaced{Figure~\ref{fig:gap_garden}}{figure}.
%
When the bird and the bee are within the same cell, the bee needs to stop flying and hide in its current location until the bird goes away. The motion of the bird is given by a Markov chain. 
%
Besides the stochastic movement of the bird, 
the weather is also stochastic and affects the robot's planning.     
%
The robot cannot pollinate a flower while raining.
%
We assume when the robot starts its task, at the leftmost cell at the bottom row, it is not raining and the probability that it will rain in the next step is $0.2$. 
%
This probability increases for the consecutive steps each time by $0.2$ until the rain starts.
%
Once the rain started, the probability for the rain to stop in the five following time steps will respectively be $0.2$, $0.4$, $0.6$, $0.8$, and $1.0$, assuming the rain has not already stopped at any of those time steps.
%
%

 We consider two scenarios for the case study. 
First, we assume that the dynamics of bee robot are deterministic. 
That is, when the robot decides to perform an action to move to a neighboring cell, its actuators will guarantee  that the robot will move to that cell after performing the action.
Second, we consider the case where actions of bee robot have probabilistic consequences. 
Specifically, the probability that the robot reaches the intended cell is $0.7$.
For each of the unintended directions except the opposite direction, the probably that the robot's actuators move the robot to that unintended direction with equal probabilities.
If the robot hits the boundary, it stays in its current cell.


Using these two scenarios, we analyze the following questions. 
\begin{enumerate}
	\item How does the choice of weight vector for scalarization affect the probabilities of satisfying various \ac{ltlf} formulas?
	\item What is the effect of stochasticity on the probabilities of satisfying various \ac{ltlf} formulas under different stochastic orders?
%	\item What effect does the choice of stochastic order have on the probabilities of satisfying various \ac{ltlf} formulas? 
\end{enumerate}
We begin with an in-depth explanation about the construction of \ac{pdfa}, the product game, and the MOMDP.  
  
\textbf{Construction of PDFA.}
% Consider the \ac{ltlf} formulas $p_1$-$p_4$ from Example~\ref{ex:ltlf-goals}. 
We first describe how the \ac{pdfa} in Figure~\ref{fig:pdfa} is generated given the preference over \ac{ltlf} formulas $p_1$-$p_4$ from Example~\ref{ex:ltlf-goals}, formulating the preferences in Figure~\ref{fig:gap_garden}.
%
Figure~\ref{fig:pdfa_experiment} shows for each of the four LTL$_f$ formula, a DFA that encodes that formula.
%
This figure also shows the \ac{pdfa} our algorithm constructs for these four formulas and the associated user preferences, consisting of the underlying DFA and the preference graph, shown respectively in Part (e) and Part (f) of this figure.

\begin{figure*}[h]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}
		\centering
		\includegraphics[scale=0.3]{pdfa_output/dfa_0.png}
		%\caption{DFA for $p_1$.}
		\caption{DFA for $p_1$: $(\neg d \wedge \neg o) \until (t \wedge \Next \Eventually ( d \vee o))$.}
		%\label{fig:underlying-dfa}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.44\textwidth}
		\centering
		\includegraphics[scale=0.3]{pdfa_output/dfa_1.png}
		%\caption{DFA for $p_2$.}
		\caption{DFA for $p_2$: $\neg t \until ((o \wedge \Next \Eventually (d \vee t)) \vee (d \wedge \Next \Eventually ( o \vee  t)))$.}
		%\label{fig:preference-graph}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.3\textwidth}
		\centering
		\includegraphics[scale=0.3]{pdfa_output/dfa_2.png}
		%\caption{DFA for $p_3$.}
		\caption{DFA for $p_3$: $(\neg d \wedge \neg o) \until (t \wedge \Always (\neg d \wedge \neg o))$.}
		%\label{fig:preference-graph}
	\end{subfigure}
	%\vspace{-20pt}
	\hfill
	\begin{subfigure}[b]{0.27\textwidth}
		\centering
		\includegraphics[scale=0.285]{pdfa_output/dfa_3.png}
		%\caption{DFA for $p_3$.}
		\caption{DFA for $p_4$: $\Always(\neg d \land \neg o \land \neg t) \lor (\Eventually o \land \Always(\neg d \land \neg t)) \lor  (\Eventually d \land \Always(\neg o \land \neg t))$.}
		%\label{fig:preference-graph}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.44\textwidth}
		\centering
		\includegraphics[scale=0.29]{pdfa_output/pdfa_dfa.png}
		\caption{The underlying DFA of the \ac{pdfa}.}
		%\label{fig:preference-graph}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.28\textwidth}
		\centering
		\includegraphics[scale=0.285]{pdfa_output/pdfa_pref_graph.png}
		\caption{The preference graph of the \ac{pdfa}.}
		
		%\label{fig:preference-graph}
	\end{subfigure}  
	% 
	\caption{\textbf{a)-d)} The DFAs for $p_1-p_4$ for the example Figure~\ref{fig:gap_garden}, which are constructed
		by our online tools, available at \url{https://akulkarni.me/prefltlf2pdfa.html}.
		%
		\textbf{e)-f)} The PDFA for the example in Figure~\ref{fig:gap_garden}, which is constructed the implementation of our algorithm for converting a preference model over \ac{ltlf} formulas into a \ac{pdfa}.}
	\label{fig:pdfa_experiment}
\end{figure*}

% 
% Recall that for this example, $\calAP = \{t, d, o\}$, and that we assumed $\Sigma = 2^\calAP$.
% %
% However, for our implementation of this case study, we set $\Sigma = \{\emptyset, \{t\}, \{o\}, \{d\} \}$ because only this subset of $2^\calAP$ is used for labeling the states of the terminating \ac{mdp} in this example, and this helps to reduce the size of the product MDP.
% %
% Generally, given  an \ac{tlmdp} $M = \langle S, A:=\bigcup_{s \in S} A_s, \mathbf{P}, s_0, s_\bot, \calAP, L \rangle$, we can always set 
% $\Sigma = \cup_{s \in S} \{L(s)\}$ instead of setting $\Sigma = 2^\calAP$.
%
The \ac{pdfa} is generated using our open-source tool\footnote{Tool for constructing \ac{pdfa} from a preference over \ac{ltlf} formulas: \url{https://akulkarni.me/prefltlf2pdfa.html}} implemented in Python3. 
%
Note that the \ac{pdfa} in this figure is the same \ac{pdfa} in Figure~\ref{fig:pdfa}, but this figure illustrates how the states $q_0$-$q_5$ in Figure~\ref{fig:pdfa} are constructed.
% 
The states in the underlying \ac{dfa} represent the formulas satisfied by any word whose trace ends in that state.
%
For instance, $\outcomes((3, 2, 3, 4)) = \{p_4\}$. This is because the first three components $3, 2, 3$ are not accepting in their respective \ac{dfa}s, but the fourth component, $4$, is an accepting state in the \ac{dfa} for $p_4$ (see Figure~\ref{fig:pdfa_experiment}). %\jf{missing reference}
% 
The states of the preference graph encode the partition of $Q$ based on the most-preferred outcomes satisfied by the states. 
% 
For example, state $(3, 6, 3, 2)$ belongs to the block $(0, 1, 0, 0)$ since the most-preferred outcomes satisfied by $(3, 6, 3, 2)$ is $\{p_2\}$. 




%We can determine the preference between any two words in $\Sigma^*$ using the \ac{pdfa}. 
Recall how the \ac{pdfa} produces a ranking over the words in $\Sigma^*$.
% 
For example, consider two paths in the \ac{mdp} $M$: A path $\rho_1$ that pollinates tulips first and then daisies, and a path $\rho_2$ that first pollinates orchids and then daisies. 
%
The trace of $\rho_1$, $\trace(\rho_1)$, induces a path that terminates in state $(4, 5, 3, 2)$ of the underlying DFA, whereas $\trace(\rho_2)$ terminates in $(3, 6, 3, 2)$. 
%
Accordingly, state $(4, 5, 3, 2)$ of the \ac{pdfa} belongs to the block of the partition represented by the vertex $(1, 0, 0, 0)$ in the preference graph, and state $(3, 6, 3, 2)$ belongs to the block represented by the vertex $(0, 1, 0, 0)$.
%
Since the preference graph has an edge from $(0, 1, 0, 0)$ to $(1, 0, 0, 0)$, it is implied that $\rho_1$ is strictly preferred over $\rho_2$.


%     	\begin{figure}
	% 	\centering
	% 	\begin{subfigure}[b]{\columnwidth}
		% 		\centering
		% 		\includegraphics[scale=0.3]{pdfa_output/dfa_0.png}
		%   %\vspace{-20pt}
		% 		%\caption{DFA for $p_1$.}
		%   \caption{DFA for $p_1$: $(\neg d \wedge \neg o) \until (t \wedge \Next \Eventually ( d \vee o))$.}
		% 		\label{fig:dfa1}
		% 	\end{subfigure}
	% 	%    \hfill
	% 	\newline
	%          \vspace{-12pt}
	% 	\begin{subfigure}[b]{\columnwidth}
		% 		\centering
		% 		\includegraphics[scale=0.3]{pdfa_output/dfa_1.png}
		%   %\vspace{-20pt}
		% 		%\caption{DFA for $p_2$.}
		%   \caption{DFA for $p_2$: $\neg t \until ((o \wedge \Next \Eventually (d \vee t)) \vee (d \wedge \Next \Eventually ( o \vee  t)))$.}
		% 		\label{fig:dfa2}
		% 	\end{subfigure}
	% 	\newline
	%  %\vspace{-12pt}
	% 	\begin{subfigure}[b]{.45\columnwidth}
		% 		\centering
		% 		\includegraphics[scale=0.3]{pdfa_output/dfa_2.png}
		%   %\vspace{-20pt}
		% 		%\caption{DFA for $p_3$.}
		%   \caption{DFA for $p_3$: $(\neg d \wedge \neg o) \until (t \wedge \Always (\neg d \wedge \neg o))$.}
		% 		\label{fig:dfa3}
		% 	\end{subfigure}
	% 	%    \hfill
	% 	%\newline
	% 	\begin{subfigure}[b]{0.45\columnwidth}
		% 		\centering
		% 		\includegraphics[scale=0.3]{pdfa_output/dfa_3.png}
		% 		%\caption{DFA for $p_4$.}
		%   \caption{DFA for $p_4$: $\Always(\neg d \land \neg o \land \neg t) \lor (\Eventually o \land \Always(\neg d \land \neg t)) \lor  (\Eventually d \land \Always(\neg o \land \neg t))$.}
		% 		\label{fig:dfa4}
		% 	\end{subfigure}
	% 	\caption{Four DFAs corresponding to \ac{ltlf} formulas $p_1$ to $p_4$ stated in Example~\ref{ex:ltlf-goals}.}
	% 	\label{fig:dfas-explicit}
	% \end{figure}

%    	\begin{figure}
	% 	\centering
	% 	\begin{subfigure}[b]{\columnwidth}
		% 		\centering
		% 		\includegraphics[scale=0.3]{pdfa_output/dfa_0.png}
		%   %\vspace{-20pt}
		% 		\caption{DFA for $p_1$.}
		%   %\caption{DFA for $p_1$: $(\neg d \wedge \neg o) \until (t \wedge \Next \Eventually ( d \vee o))$.}
		% 		\label{fig:dfa1}
		% 	\end{subfigure}
	% 	%    \hfill
	% 	\newline
	%          \vspace{-12pt}
	% 	\begin{subfigure}[b]{\columnwidth}
		% 		\centering
		% 		\includegraphics[scale=0.3]{pdfa_output/dfa_1.png}
		%   \vspace{-20pt}
		% 		\caption{DFA for $p_2$.}
		%   %\caption{DFA for $p_2$: $\neg t \until ((o \wedge \Next \Eventually (d \vee t)) \vee (d \wedge \Next \Eventually ( o \vee  t)))$.}
		% 		\label{fig:dfa2}
		% 	\end{subfigure}
	% 	\newline
	%  \vspace{-12pt}
	% 	\begin{subfigure}[b]{.45\columnwidth}
		% 		\centering
		% 		\includegraphics[scale=0.3]{pdfa_output/dfa_2.png}
		%   \vspace{-20pt}
		% 		\caption{DFA for $p_3$.}
		%   %\caption{DFA for $p_3$: $(\neg d \wedge \neg o) \until (t \wedge \Always (\neg d \wedge \neg o))$.}
		% 		\label{fig:dfa3}
		% 	\end{subfigure}
	% 	%    \hfill
	% 	%\newline
	%  \vspace{-12pt}  
	% 	\begin{subfigure}[b]{0.45\columnwidth}
		% 		\centering
		% 		\includegraphics[scale=0.3]{pdfa_output/dfa_3.png}
		%   \vspace{-20pt}
		% 		\caption{DFA for $p_4$.}
		%   %\caption{DFA for $p_4$: $\Always(\neg d \land \neg o \land \neg t) \lor (\Eventually o \land \Always(\neg d \land \neg t)) \lor  (\Eventually d \land \Always(\neg o \land \neg t))$.}
		% 		\label{fig:dfa4}
		% 	\end{subfigure}
	
	% 	\caption{Four DFAs corresponding to \ac{ltlf} formulas $p_1$ to $p_4$ stated in Example~\ref{ex:ltlf-goals}.}
	% 	\label{fig:dfas-explicit}
	% \end{figure}


%     	\begin{figure}
	% 	\centering
	% 		\centering
	% 		\includegraphics[width=\linewidth]{pdfa_output/dfas.png}
	% 	\caption{Four DFAs corresponding to \ac{ltlf} formulas $p_1$ to $p_4$ stated in Example~\ref{ex:ltlf-goals}.}
	% 	\label{fig:dfas-explicit}
	% \end{figure}


% \begin{figure*}[t]
	% 	\centering
	% 	\begin{subfigure}[b]{0.55\textwidth}
		% 		\centering
		% 		\includegraphics[scale=0.3]{pdfa_output/pdfa_dfa.png}
		% 		\caption{The underlying DFA of the \ac{pdfa}.}
		% 		\label{fig:underlying-dfa}
		% 	\end{subfigure}
	% 	\hfill
	% 	\begin{subfigure}[b]{0.35\textwidth}
		% 		\centering
		% 		\includegraphics[scale=0.3]{pdfa_output/pdfa_pref_graph.png}
		% 		\caption{The preference graph corresponding to the \ac{pdfa}.}
		% 		\label{fig:preference-graph}
		% 	\end{subfigure}
	%        %
	
	% 	% 
	% 	\caption{PDFA for the example in Figure~\ref{fig:gap_garden}. The \ac{pdfa} constructed by our algorithm for the LTL$_f$ formulas and the preference over them. }
	% 	\label{fig:pdfa-explicit}
	% \end{figure*}

% \begin{figure*}[t]
% 	\centering
% 	\begin{subfigure}[b]{0.24\textwidth}
% 		\centering
% 		\includegraphics[scale=0.3]{pdfa_output/dfa_0.png}
% 		%\caption{DFA for $p_1$.}
% 		\caption{DFA for $p_1$: $(\neg d \wedge \neg o) \until (t \wedge \Next \Eventually ( d \vee o))$.}
% 		%\label{fig:underlying-dfa}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[b]{0.44\textwidth}
% 		\centering
% 		\includegraphics[scale=0.3]{pdfa_output/dfa_1.png}
% 		%\caption{DFA for $p_2$.}
% 		\caption{DFA for $p_2$: $\neg t \until ((o \wedge \Next \Eventually (d \vee t)) \vee (d \wedge \Next \Eventually ( o \vee  t)))$.}
% 		%\label{fig:preference-graph}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[b]{0.3\textwidth}
% 		\centering
% 		\includegraphics[scale=0.3]{pdfa_output/dfa_2.png}
% 		%\caption{DFA for $p_3$.}
% 		\caption{DFA for $p_3$: $(\neg d \wedge \neg o) \until (t \wedge \Always (\neg d \wedge \neg o))$.}
% 		%\label{fig:preference-graph}
% 	\end{subfigure}
% 	%\vspace{-20pt}
% 	\hfill
% 	\begin{subfigure}[b]{0.27\textwidth}
% 		\centering
% 		\includegraphics[scale=0.285]{pdfa_output/dfa_3.png}
% 		%\caption{DFA for $p_3$.}
% 		\caption{DFA for $p_4$: $\Always(\neg d \land \neg o \land \neg t) \lor (\Eventually o \land \Always(\neg d \land \neg t)) \lor  (\Eventually d \land \Always(\neg o \land \neg t))$.}
% 		%\label{fig:preference-graph}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[b]{0.44\textwidth}
% 		\centering
% 		\includegraphics[scale=0.29]{pdfa_output/pdfa_dfa.png}
% 		\caption{The underlying DFA of the \ac{pdfa}.}
% 		%\label{fig:preference-graph}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[b]{0.28\textwidth}
% 		\centering
% 		\includegraphics[scale=0.285]{pdfa_output/pdfa_pref_graph.png}
% 		\caption{The preference graph of the \ac{pdfa}.}
		
% 		%\label{fig:preference-graph}
% 	\end{subfigure}  
% 	% 
% 	\caption{\textbf{a)-d)} The DFAs for $p_1-p_4$ for the example Figure~\ref{fig:gap_garden}, which are constructed
% 		by our online tools, available at \url{https://akulkarni.me/prefltlf2pdfa.html}.
% 		%
% 		\textbf{e)-f)} The PDFA for the example in Figure~\ref{fig:gap_garden}, which is constructed the implementation of our algorithm for converting a preference model over \ac{ltlf} formulas into a \ac{pdfa}.}
% 	\label{fig:pdfa_experiment}
% \end{figure*}



%\subsection{Case 1: Deterministic Action Transitions but Uncertain Environments}

 \textbf{Construction of Product Game.} 
For scenario 1 where the robot's actions have deterministic outcomes, the constructed MDP has $10,460$ states and $280,643$ transitions. 
The product MDP had $36,649$ states and $946,467$ transitions.
For scenario 2 where the robot's actions have probabilistic outcomes, the constructed MDP has the same number of states but $779,396$ transitions. 
The product MDP had $36,649$ states and $2,628,508$ transitions.
The MDP and the product MDP construction together required about $5$ seconds for each scenario. 

\deleted{
%
For the case when the robot's actions have deterministic outcomes,	the constructed MDP   has $10,460$ states and $280,643$ transitions (its transition function has $280,643$ entries with non-zero probabilities).
%
It took $39.06$ seconds for our program to construct the MDP. 
%
The product MDP had $36,649$ states and $946,467$ transitions.
%
The average construction times for the product MDP over $10$ constructions for each of the weak stochastic order, strong stochastic order, and weak* stochastic order were respectively $238.78$, $238.57$, and $238.76$ seconds.
%
}


Given the preference described in Fig.~\ref{fig:pdfa}, we employ linear scalarization methods to solve the \ac{momdp}.  
Specifically, given a weight vector  $\mathbf{w} \in [0, 1]^N$ , we compute the nondominated policy $\mu_{\mathbf{w}}$, by first setting $V_{\mathbf{w}}(x) = \sum_{1 \leq i \leq N: x \in Z_i} \mathbf{w}[i] $ for each goal state $x \in X_G$, and then by solving the following Bellman equation for the values of  the non-goal states $x \in X \setminus X_G$:
%\hr{I think it might be better to use $V_{\mathbf{w}}(x) = \sum_{1 \leq i \leq N: x \in Z_i}$ instead of $V_{\mathbf{w}}(x) = \sum_{1 \leq i \leq N, x \in Z_i}$ because the latter might be confused that the subscript imposes to conditions. We can also consider $V_{\mathbf{w}}(x) = \sum_{1 \leq i \leq N \text{s.t. } x \in Z_i}$}\jf{agree with the first one.}
%
\begin{equation}
	%V_{\mathbf{w}}(x) = \max_{a \in A_x} \sum_{x' \in X} \mathbf{T}(x, a, x')V_{\mathbf{w}}(x'), \forall x \in X \setminus X_G.
	V_{\mathbf{w}}(x) = \max_{a \in A_x} \sum_{x' \in X} \mathbf{T}(x, a, x')V_{\mathbf{w}}(x').
\end{equation}
%
%
The policy for those states is recovered from $V_{\mathbf{w}}(x)$ as
\begin{equation}
	%\mu_{\mathbf{w}}(x) = \argmax_{a \in A_x} \sum_{x' \in X} \mathbf{T}(x, a, x')V_{\mathbf{w}}(x'), \forall x\in X \setminus X_G.
	\mu_{\mathbf{w}}(x) = \argmax_{a \in A_x} \sum_{x' \in X} \mathbf{T}(x, a, x')V_{\mathbf{w}}(x').
\end{equation}
%
For each of the three stochastic orderings $\mathfrak{E} \in \{\mathfrak{E}_{st}, \mathfrak{E}_{wk}, \mathfrak{E}_{wk*}\}$, we randomly generated $1,000$ weight vectors and used each one of them to compute a Pareto optimal policy for the MOMDP.  


\added{
We first observe that our results are consistent with the findings of Theorem~\ref{thm:pareto-weakstochastic}.
That is, no policy in the set of $1,000$ sampled polices is $\mathfrak{E}$-stochastic dominated by any other policy in that set.
}

\deleted{
For each stochastic orderings $\mathfrak{E}$, the $1,000$ computed Pareto-optimal policies are expected to be $\mathfrak{E}$-nondominated policies.
%
From the result, it is noted that for each stochastic orderings $\mathfrak{E}$, none of those $1,000$ computed polices were $\mathfrak{E}$-stochastic dominated by the other polices. This is expected due to Theorem~\ref{thm:pareto-weakstochastic}.
}
%

Next, we provide more detailed analysis for weak-stochastic non-dominated policies. 
\added{The analysis for other types of orders is similar.}
Recall from Table~\ref{tab:objectives} that the objectives for the weak-stochastic ordering are $\{p_1\}$, $\{p_1, p_2\}$, and
$\{p_1, p_3\}$.
%
Since it is difficult to illustrate the 3D Pareto front, we select a set of policies with similar probabilities (approximately 0.24) of satisfying $p_1$ and then plot the values of these policies for the objectives $\{p_1, p_2\}$ and $\{p_1, p_3\}$. Figure~\ref{fig:case_study_pareto_front} shows the values of those  policies for the objectives $\{p_1, p_2\}$ and $\{p_1, p_3\}$. 
%
This figure shows that none of those policies weak-stochastic dominates each other. %(consider that all those $1,000$ policies satisfy the objective $\{p_1, p_2, p_3, p_4\}$) with probability $1.0$.

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.35]{figures/Pareto_Front_327rows_from_1000rows.png}
	\caption{
		The probabilities of satisfying objectives $\{p_1, p_2\}$ and $\{p_1, p_3\}$ by the computed policies for weak-stochastic ordering who satisfy the objective $\{p_1\}$ with probability $0.2406$. 
	}
	\label{fig:case_study_pareto_front}
\end{figure}

%

%

%           	    \begin{table}[h!]
	%    \setlength{\tabcolsep}{0.2em}
	%   \centering
	%   \begin{tabular}{cccc}
		%   \hline \hline
		%    & \scriptsize     Weight Vector & \scriptsize  Value Vector & \scriptsize  Prob. of individual outcomes \\ 
		%    %   \multicolumn{4}{l}{\ \tiny [$\{p_1\}, \{p_1, p_2\}, \{p_1, p_3\}, \{p_1, p_2, p_3, p_4\}$] \ \ \ \ \ \ \ \ \ \ \ \ \ \  \tiny [$p_1, p_2, p_3, p_4$]}\\
		% %      \multicolumn{4}{l}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \tiny [$\{p_1\}, \{p_1, p_2\}, \{p_1, p_3\}, \{p_1, p_2, p_3, p_4\}$]}\\[1ex]
		%   %\scriptsize  & [\{p_1\}, \{p_1. p_2\}, \{p_1, p_3 \}, \{p_1, p_2, p_3, p_4 \} ] & \scriptsize Policy \scriptsize Value Vector & \scriptsize Preferences Probabilities \\ [1ex]
		%   \hline
		%   %\scriptsize [0.157, 0.463, 0.272, 0.108] & \scriptsize [0.118, 0.781, 0.321, 1.0] & \scriptsize [0.118, 0.663, 0.203, 0.016] \\
		%    % Row 156
		%  \scriptsize 1 &  \scriptsize [0.39, 0.35, 0.10, 0.16] & \scriptsize 	[0.11, 0.80, 0.29, 1.0] & \scriptsize [0.11, 0.69, 0.18, 0.02] \\
		%   % Row 467
		%  \scriptsize 2 &  \scriptsize [0.27, 0.32, 0.15, 0.26] & \scriptsize 	[0.15, 0.73, 0.40, 1.0] & \scriptsize [0.15, 0.58, 0.25, 0.02] \\
		%   % Row 725
		%   \scriptsize 3 &  \scriptsize [0.16, 0.37, 0.23, 0.24] & \scriptsize 	[0.20, 0.56, 0.63, 1.0] & \scriptsize [0.20, 0.36, 0.43, 0.01] \\
		%   % Row 809
		%   \scriptsize 4 &  \scriptsize [0.11, 0.44, 0.30, 0.16] & \scriptsize 	[0.17, 0.64, 0.53, 1.0] & \scriptsize [0.17, 0.47, 0.35, 0.01] \\
		%   % Row 790
		%   \scriptsize 5 &  \scriptsize [0.12, 0.47, 0.28, 0.13] & \scriptsize 	[0.07, 0.87, 0.19, 1.0] & \scriptsize [0.07, 0.80, 0.12, 0.01] \\
		%   % Row 118
		%   \scriptsize 6 &  \scriptsize [0.42, 0.32, 0.22, 0.04] & \scriptsize 	[0.24, 0.43, 0.80, 1.0] & \scriptsize [0.24, 0.19, 0.56, 0.01] \\
		%   % Row 204
		%   \scriptsize 7 &  \scriptsize [0.37, 0.19, 0.30, 0.14] & \scriptsize 	[0.24, 0.25, 0.98, 1.0] & \scriptsize [0.24, 0.01, 0.74, 0.01] \\   
		%   % Row 684
		%   \scriptsize 8 &  \scriptsize [0.18, 0.33, 0.32, 0.17] & \scriptsize 	[0.24, 0.31, 0.92, 1.0] & \scriptsize [0.24, 0.06, 0.68, 0.02] \\
		%    % Row 18
		%    \scriptsize 9 &  \scriptsize [0.60, 0.17, 0.04, 0.19] & \scriptsize 	[0.24, 0.43, 0.79, 1.0] & \scriptsize [0.24, 0.19, 0.55, 0.01] \\
		%    % Row 927
		%    \scriptsize 10 &  \scriptsize [0.05, 0.45, 0.42, 0.08] & \scriptsize 	[0.24, 0.40, 0.83, 1.0] & \scriptsize [0.24, 0.16, 0.59, 0.01] \\
		%   \end{tabular}
	%       \caption{Ten weak-stochastic nondominated polices computed by our algorithm for the Garden case study. 
		%       %
		%   }
	%   \label{tbl:nondom_policies}
	%   \end{table}
\begin{table*}[h!]
	\setlength{\tabcolsep}{0.4em}
	\centering
	\begin{tabular}{cccc}
		\hline \hline
		& \scriptsize     Weight Vector & \scriptsize \makecell{Value Vector \\ $[\{p_1\}, \{p_1, p_2\}, \{p_1, p_3\}]$} & \scriptsize  \makecell{Prob. of individual outcomes \\ $[p_1, p_2, p_3, p_4]$} \\ 
		%& \tiny      & \tiny  $[\{p_1\}, \{p_1, p_2\}, \{p_1, p_3\}]$ & \tiny \renewcommand{\arraystretch}{1} 
		% \\ 
		%   \multicolumn{4}{l}{\ \tiny [$\{p_1\}, \{p_1, p_2\}, \{p_1, p_3\}, \{p_1, p_2, p_3, p_4\}$] \ \ \ \ \ \ \ \ \ \ \ \ \ \  \tiny [$p_1, p_2, p_3, p_4$]}\\
		%      \multicolumn{4}{l}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \tiny [$\{p_1\}, \{p_1, p_2\}, \{p_1, p_3\}, \{p_1, p_2, p_3, p_4\}$]}\\[1ex]
		%\scriptsize  & [\{p_1\}, \{p_1. p_2\}, \{p_1, p_3 \}, \{p_1, p_2, p_3, p_4 \} ] & \scriptsize Policy \scriptsize Value Vector & \scriptsize Preferences Probabilities \\ [1ex]
		\hline
		%\scriptsize [0.157, 0.463, 0.272, 0.108] & \scriptsize [0.118, 0.781, 0.321, 1.0] & \scriptsize [0.118, 0.663, 0.203, 0.016] \\
		% Row 156
		\scriptsize 1 &  \scriptsize [0.466, 0.412, 0.122] & \scriptsize 	[0.110, 0.799, 0.291] & \scriptsize [0.110, 0.689, 0.181, 0.020] \\
		% Row 467
		\scriptsize 2 &  \scriptsize [0.363, 0.438, 0.199] & \scriptsize 	[0.146, 0.726, 0.395] & \scriptsize [0.146, 0.580, 0.249, 0.025] \\
		% Row 725
		\scriptsize 3 &  \scriptsize [0.207, 0.484, 0.309] & \scriptsize 	[0.201, 0.558, 0.633] & \scriptsize [0.201, 0.357, 0.432, 0.01] \\
		% Row 809
		\scriptsize 4 &  \scriptsize [0.134, 0.519, 0.347] & \scriptsize 	[0.173, 0.638, 0.527] & \scriptsize [0.173, 0.465, 0.354, 0.008] \\
		% Row 790
		\scriptsize 5 &  \scriptsize [0.141, 0.541, 0.318] & \scriptsize 	[0.068, 0.874, 0.187] & \scriptsize [0.068, 0.806, 0.119, 0.007] \\
		% Row 118
		\scriptsize 6 &  \scriptsize [0.434, 0.339, 0.227] & \scriptsize 	[0.241, 0.427, 0.798] & \scriptsize [0.241, 0.186, 0.557, 0.016] \\
		% Row 204
		\scriptsize 7 &  \scriptsize [0.428, 0.223, 0.349] & \scriptsize 	[0.239, 0.250, 0.980] & \scriptsize [0.239, 0.011, 0.741, 0.009] \\   
		% Row 684
		\scriptsize 8 &  \scriptsize [0.213, 0.395, 0.392] & \scriptsize 	[0.240, 0.307, 0.925] & \scriptsize [0.240, 0.067, 0.685, 0.008] \\
		% Row 18
		\scriptsize 9 &  \scriptsize [0.742, 0.208, 0.050] & \scriptsize 	[0.240, 0.432, 0.787] & \scriptsize [0.240, 0.192, 0.547, 0.021] \\
		% Row 927
		\scriptsize 10 &  \scriptsize [0.057, 0.488, 0.455] & \scriptsize 	[0.240, 0.398, 0.831] & \scriptsize [0.240, 0.158, 0.591, 0.011] \\
		\hline
	\end{tabular}
	\caption{Ten weak-stochastic nondominated polices computed by our algorithm for the Garden case study. 
		%
	}
	\label{tbl:nondom_policies}
\end{table*} 
Table~\ref{tbl:nondom_policies} shows $10$ out of those $1,000$ weight vectors along with the value vectors of the weak-stochastic non-dominated polices computed for those weight vectors and the corresponding probabilities those polices assign to the four preferences $p_1$ through $p_4$.
%
\added{The third column shows the multi-objective value vector of each computed policy. }
%
For each policy, the last column shows a probability distribution over individual outcomes $p_1,\ldots, p_4$ indicating the probabilities of satisfying those formulas (in that order), given the computed policy. 
%
\added{These probabilities are determined by solving a system of equations based on subsets of outcomes. For example, take the first weight vector which yields the value $[0.110, 0.799, 0.291]$. In this case, the system of equations is as follows: let $x_i$ represent the probability that $p_i$ is satisfied. The equations are $x_1 = 0.110$, $x_1 + x_2 = 0.799$, $x_1 + x_3 = 0.291$, and $x_1 + x_2 + x_3 + x_4 = 1.0$.}
%
\deleted{The third column shows the multi-objective value vector of each computed policy. It is noted that
none of those value vectors dominates any other value vector.}


\textbf{Effect of Weight Vector.}
\added{The proposed synthesis approach implicitly manages a trade-off between the preference of satisfying an outcome with the likelihood that it can enforce its satisfaction given the uncertainties.}
%
\added{For instance, on} rows $6$ and $9$ of \replaced{Table 2, we observe that}{this table we show that} even if the weight assigned to the most preferred outcome, $p_1$, is significantly higher than the weights assigned to the other preferences, the probability that $p_1$ to be satisfied is still less than $0.25$. 
%
\replaced{This is due to the fact that robot needs a minimum of 12 steps to satisfy $p_1$. As a result,  }
{This is justified by the fact that the robot's battery capacity supports the robot for only $12$ time steps and thus }
to achieve $p_1$, the robot must not be stopped by the bird and not encounter rain when it reaches a cell to do pollination.
\added{Since} the probability to satisfy these conditions given the environment dynamics is less than $0.25$, \added{the probability of satisfying $p_1$ under any strategy regardless of weight is smaller than $0.25$}.
%

\added{
On the other hand, consider the eighth and tenth rows in Table 2, where the subsets $\{p_1, p_2\}$ and $\{p_1, p_3\}$ have almost equal weights in the weight vector.
We observe that the value assigned to $\{p_1, p_3\}$ (which is the probability of satisfying either $p_1$ or $p_3$) is significantly higher than the value of $\{p_1, p_2\}$. 
This is because satisfying $p_1$ implies $p_3$ but no such relation holds between $p_1$ and $p_2$. 
When the weight vectors do not explicitly favor one subset over the other, the synthesized policy implicitly prioritizes the subset $\{p_1, p_3\}$ over $\{p_1, p_2\}$.
In the first case, policy can ensure $p_3$ is satisfied with a high probability since it is 7 steps away from robot's initial position. 
Thereafter, an attempt to satisfy $p_1$ could be made to satisfy a better outcome.
However, in the second case, the policy must decide between satisfying $p_1$ or $p_2$ since both cannot be achieved simultaneously given the time constraint. 
Here, the implicit trade-off occurs between satisfying only $p_2$ with a high probability against a slightly lower probability of satisfying $p_3$ but a prospect of satisfying $p_1$ after that.
}
 
 

\deleted{
	The probability of $p_4$ to be satisfied in any entry of this table is very small, regardless of the weight vector. 
	This is because $p_4$ has the lowest priority, and any policy would prefer to satisfy other preferences who are assigned higher priorities.
}


\deleted{
Although the objectives $\{p_1, p_2\}$ and $\{p_1, p_3\}$ in the eighth and the tenth rows are treated almost equally by the weight vector in terms of importance, the probability that the later to be satisfied is significantly bigger than the probability of the former to be satisfied. 
This is because the objective $\{p_1 \}$ contains the preference with the highest priority and that those two rows assign a very high weight to this objective, forcing the policy to try to satisfy $p_1$.
Further, by attempting to perform $p_1$, the robot has the chance to accomplish $p_3$ within the same attempt, even if it fails to accomplish $p_1$. % \jf{do you mean $p_2$? or it fails to accomplish $p_1$ with a high probability?}
%  \hrm{I think the text I have written is correct. See Figure~\ref{fig:gap_garden} for the meaning of $p_1$ through $p_4$.}
%
More precisely, if in attempting to perform the task $p_1$---first tulips and then at least one out of daisies and orchids---the robot succeeds to pollinate the tulips but fails to pollinate the daisies and orchids, then it has already accomplished $p_3$, even though it has failed in accomplishing what it was aiming for---$p_1$.
}



%   \begin{table}[h!]
	%    \setlength{\tabcolsep}{0.2em}
	%   \centering
	%   \begin{tabular}{cccccccc}
		%   \hline \hline
		%    & \scriptsize  Weight Vector & \scriptsize  Value Vector  & \scriptsize  Prob. of individual outcomes 
		%    & \scriptsize  Value Vector  & \scriptsize  Prob. of individual outcomes 
		%    & \scriptsize  Value Vector & \scriptsize  Prob. of individual outcomes 
		%    \\ 
		%    & \scriptsize  (weak order) & \scriptsize (weak order)  & \scriptsize (weak* order) & \scriptsize (weak* order) & \scriptsize (strong order) & \scriptsize (strong order) \\
		%    %   \multicolumn{4}{l}{\ \tiny [$\{p_1\}, \{p_1, p_2\}, \{p_1, p_3\}, \{p_1, p_2, p_3, p_4\}$] \ \ \ \ \ \ \ \ \ \ \ \ \ \  \tiny [$p_1, p_2, p_3, p_4$]}\\
		% %      \multicolumn{4}{l}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \tiny [$\{p_1\}, \{p_1, p_2\}, \{p_1, p_3\}, \{p_1, p_2, p_3, p_4\}$]}\\[1ex]
		%   %\scriptsize  & [\{p_1\}, \{p_1. p_2\}, \{p_1, p_3 \}, \{p_1, p_2, p_3, p_4 \} ] & \scriptsize Policy \scriptsize Value Vector & \scriptsize Preferences Probabilities \\ [1ex]
		%   \hline
		%   %\scriptsize [0.157, 0.463, 0.272, 0.108] & \scriptsize [0.118, 0.781, 0.321, 1.0] & \scriptsize [0.118, 0.663, 0.203, 0.016] \\
		%    % Row 156
		%  \scriptsize 1 &  \scriptsize [0.39, 0.35, 0.10, 0.16] & \scriptsize [0.11, 0.80, 0.29, 1.0] & \scriptsize [0.11, 0.69, 0.18, 0.02]  & \scriptsize [0.0, 0.99, 0.0, 0.99] & \scriptsize [0.0, 0.99, 0.0, 0.01] & \scriptsize [0.07, 0.87, 0.19, 0.997] & \scriptsize [0.07, 0.80, 0.12, 0.01] \\
		%   % Row 467
		%  \scriptsize 2 &  \scriptsize [0.27, 0.32, 0.15, 0.26] & \scriptsize [0.15, 0.73, 0.40, 1.0] & \scriptsize [0.15, 0.58, 0.25, 0.02] & \scriptsize [0.0, 0.99, 0.0, 0.99] & \scriptsize [0, 0.99, 0, 0.01] & \scriptsize [0.139, 0.711, 0.452, 0.99] & \scriptsize [, , ,] \\
		%   % Row 725
		%   \scriptsize 3 &  \scriptsize [0.16, 0.37, 0.23, 0.24] & \scriptsize [0.20, 0.56, 0.63, 1.0] & \scriptsize [0.20, 0.36, 0.43, 0.01] & \scriptsize [0.0, 0.99, 0.0, 0.99] & \scriptsize [0.0, 0.99, 0.0, 0.01] & \scriptsize [0.175, 0.630, 0.537, 0.992] & \scriptsize [, , ,] \\
		%   % Row 809
		%   \scriptsize 4 &  \scriptsize [0.11, 0.44, 0.30, 0.16] & \scriptsize [0.17, 0.64, 0.53, 1.0] & \scriptsize [0.17, 0.47, 0.35, 0.01] & \scriptsize [0.0, 0.92, 0.11, 0.99] & \scriptsize [0.04, 0.88, 0.7, 0.01] & \scriptsize [0.176, 0.630, 0.537, 0.992] & \scriptsize [, , ,] \\
		%   % Row 790
		%   \scriptsize 5 &  \scriptsize [0.12, 0.47, 0.28, 0.13] & \scriptsize [0.07, 0.87, 0.19, 1.0] & \scriptsize [0.07, 0.80, 0.12, 0.01] & \scriptsize [0.0, 0.99, 0.0, 0.99] & \scriptsize [0.0, 0.99, 0.0, 0.01] & \scriptsize [0.077, 0.850, 0.222, 0.996] & \scriptsize [, , ,]  \\
		%   % Row 118
		%   \scriptsize 6 &  \scriptsize [0.42, 0.32, 0.22, 0.04] & \scriptsize [0.24, 0.43, 0.80, 1.0] & \scriptsize [0.24, 0.19, 0.56, 0.01] & \scriptsize [0.0, 0.92, 0.11, 0.99] & \scriptsize [0.03, 0.89, 0.7, 0.01] & \scriptsize [0.241, 0.427, 0.799, 0.985] & \scriptsize [, , ,] \\
		%   % Row 204
		%   \scriptsize 7 &  \scriptsize [0.37, 0.19, 0.30, 0.14] & \scriptsize [0.24, 0.25, 0.98, 1.0] & \scriptsize [0.24, 0.01, 0.74, 0.01] & \scriptsize [0.0, 0.24, 0.99, 0.99] & \scriptsize [0.24, 0.0, 0.75, 0.01] & \scriptsize [0.240, 0.250, 0.980, 0.991] & \scriptsize [, , ,]  \\   
		%   % Row 684
		%   \scriptsize 8 &  \scriptsize [0.18, 0.33, 0.32, 0.17] & \scriptsize [0.24, 0.31, 0.92, 1.0] & \scriptsize [0.24, 0.06, 0.68, 0.02] & \scriptsize [0.0, 0.31, 0.92, 0.99] & \scriptsize [0.24, 0.06, 0.69, 0.01] & \scriptsize [0.241, 0.307, 0.925, 0.992] & \scriptsize [, , ,]  \\
		%    % Row 825
		%    \scriptsize 9 &  \scriptsize [0.10, 0.40, 0.21, 0.29] & \scriptsize [0.0, 0.99, 0.0, 1.0] & \scriptsize [0.0, 0.99, 0.0, 0.01] & \scriptsize [0.0, 0.99, 0.0, 0.99] & \scriptsize [0.0, 0.99, 0.0, 0.01] & \scriptsize [0.000, 0.998, 0.000, 0.998] & \scriptsize [, , ,]  \\
		%    % Row 927
		%    \scriptsize 10 &  \scriptsize [0.05, 0.45, 0.42, 0.08] & \scriptsize [0.24, 0.40, 0.83, 1.0] & \scriptsize [0.24, 0.16, 0.59, 0.01] & \scriptsize [0.0, 0.38, 0.85, 0.99] & \scriptsize [0.24, 0.14, 0.61, 0.01] & \scriptsize [0.241, 0.383, 0.848, 0.990] & \scriptsize [, , ,]  \\
		%   \end{tabular}
	%       \caption{Ten weak-stochastic nondominated polices computed by our algorithm for the Garden case study. 
		%       %
		%   }
	%   \label{tbl:nondom_policies}
	%   \end{table}

%Although the objectives $\{p_1, p_2\}$ and $\{p_1, p_3\}$ in the eighth and the tenth rows are treated almost equally by the weight vector in terms of importance, the probability that the later to be satisfied is significantly bigger than the probability of the former to be satisfied. 
%\ak{Insight Stmt: This is because the objective $\{p_1 \}$ contains the preference with the highest priority and that those two rows assign a very high weight to this objective, forcing the policy to try to satisfy $p_1$.} 
%Further, by attempting to perform $p_1$, the robot has the chance to accomplish $p_3$ within the same attempt, even if it fails to accomplish $p_1$. % \jf{do you mean $p_2$? or it fails to accomplish $p_1$ with a high probability?}
%%  \hrm{I think the text I have written is correct. See Figure~\ref{fig:gap_garden} for the meaning of $p_1$ through $p_4$.}
%%
%More precisely, if in attempting to perform the task $p_1$---first tulips and then at least one out of daisies and orchids---the robot succeeds to pollinate the tulips but fails to pollinate the daisies and orchids, then it has already accomplished $p_3$, even though it has failed in accomplishing what it was aiming for---$p_1$.

%\subsection{Case 2: Introducing Stochastic    Robot Dynamics}

\deleted{
The MDP for this variant has the same number of states, $10,460$, but it has more transitions, $779,396$, which is due to  the stochasticity in   robot's dynamics.
%
We consider all the three types of stochastic orderings.
%
The MDP construction time for weak-stochastic ordering, strong-stochastic ordering, and weak*-stochastic ordering were respectively $205.92$, $203,43$
and $238.83$ seconds. The construction time of the product MDP for these three stochastic ordering types were respectively $1,088.58$, $1,088.59$, and $1,089.02$ seconds.
}

%The MDP construction time for this case was $205.92$ seconds and it took $1,082.23$ seconds to make the product MDP.
% We again computed $100$ weak-stochastic nondominated policies. 
%

 \textbf{Effect of Stochasticity.}
As the stochasticity   increases, the synthesized policy becomes more conservative, assuming the same stochastic ordering and weight vector. 
Let us compare the policies synthesized under each stochastic order for scenario 1 and scenario 2 assuming uniform weights.
Under weak-stochastic ordering with the weight vector $[0.3333, 0.3333, 0.3334]$, the non-stochastic variant achieves the following probabilities: $[p_1: 0.241, p_2: 0.053, p_3: 0.699, p_4: 0.007]$, while in the stochastic variant, the probabilities shift to $[p_1: 0.008, p_2: 0.821, p_3: 0.120, p_4: 0.051]$. 
The key insight here is that the increase in stochasticity results in significant decrease in the probability of satisfying $p_3$ and by extension $p_1$, which flips the decision of the policy when trading-off between low probability of satisfying $p_3$ and then $p_1$ against high probability of satisfying only $p_2$.
 

A similar pattern emerges under strong-stochastic ordering with the weight vector $[0.25, 0.25, 0.25, 0.25]$, where the non-stochastic case yields probabilities $[p_1: 0.241, p_2: 0.053, p_3: 0.699, p_4: 0.007]$, with a high probability to satisfy $p_3$, and the stochastic case results in $[p_1: 0.002, p_2: 0.931, p_3: 0.026, p_4: 0.041]$, again with a high probability to satisfy $p_2$ instead.


Lastly, under weak*-stochastic ordering and the same weight vector, the non-stochastic probabilities are $[p_1: 0.241, p_2: 0.053, p_3: 0.699, p_4: 0.007]$, while the stochastic case shows $[p_1: 0.000, p_2: 0.953, p_3: 0.007, p_4: 0.040]$, with a strong emphasis on satisfying $p_2$ at the cost of other objectives.


\deleted{
Due to the stochasticity in the robot's dynamic, for each kind of stochastic ordering, we expect the policy computed for a specific weight vector to perform ``poorer'' than a policy computed for the same weight vector of Case 1.
%
We first compare the two polices for weak-stochastic ordering, given the weight vector $[0.3333, 0.3333, 0.3334]$.
%
The probabilities of the preferences to be satisfied for the variant without stochasticity were $[p_1: 0.241, p_2: 0.053, p_3:0.699, p_4: 0.007]$, while those probabilities for the variant with stochasticity were $[p_1: 0.008, p_2: 0.821, p_3:0.120, p_4: 0.051]$.
%
While the former policy yields a higher probability of achieving $p_3$, the latter policy puts most of its efforts to satisfy $p_2$ and has a very low probability (close to 0) to satisfy the most preferred goal $p_1$.
%
Similar observation is made for strong-stochastic ordering using the weight vector $[0.25, 0.25, 0.25, 0.25]$.
%
The probabilities of the preferences to be satisfied for the variant without stochasticity were $[p_1: 0.241, p_2: 0.053, p_3: 0.699, p_4: 0.007]$, while those probabilities for the variant with stochasticity were $[p_1: 0.002, p_2: 0.931, p_3: 0.026, p_4: 0.041]$. 
% This result is similar to the case with weak-stochastic ordering: The robot satisfies $p_2$ with a much higher probability than $p_3$ when stochastic dynamics is introduced.
%
%
Lastly, for weak*-stochastic ordering, we have three  objectives $\{p_1, p_2\}$, $\{p_1, p_3\}$, $\{p_1, p_2, p_3\}$ (after removing the empty set and 
the set  $\{p_1, p_2, p_3, p_4\}$). Given the weight vector $[0.3333, 0.3333, 0.3334]$, % and compare the two policies for weak*-stochastic ordering for the example with and without stochasticity, respectively.
% %\jf{what is being compared: weak* or strong? }
% %
the probabilities of the preferences to be satisfied for the variant without stochasticity were $[p_1: 0.241, p_2: 0.053, p_3: 0.699, p_4: 0.007]$, while those probabilities for the variant with stochasticity were $[p_1: 0.000, p_2: 0.953, p_3: 0.007, p_4: 0.040]$. 
% 
}


%\textbf{Effect of Choice of Stochastic Order.}
\deleted{
Given the \replaced{uniform}{same} weight vector but different stochastic orderings, we observed that the probability of satisfying $p_2$ in the stochastic variant is much larger ($\approx$ 16 times more likely)  than that of the deterministic variant. This result is mainly due to the difficulty in reaching tulips given the coupled inherent stochastic dynamics and uncertain environmental factors (clouds and the bird). Because the chance of reaching tulips is very small, the probability of satisfying $p_1$ or $p_3$ -- both require tulips to be visited --- are equally small. 
\ak{Insight Stmt: As a result, the preference-based planner (across all three stochastic orders)  satisfies $p_2$ with a much higher probability since $p_2$ only requires two flower types to be pollinated.}
This experimental comparison demonstrates the flexibility of preference-based planners to adjust the goal based on changes in the system and environment dynamics.
}

% In all these three comparisons, the probability of satisfying an outcome $p_i$ by all the three kinds of stochastic orderings for the case without stochasticity in the robot's dynamic is the same.
% %
% This can be attributed to connection between the objectives of the \ac{momdp}s under these three kinds of stochastic orderings for this specific example and that the weight vectors for all these three comparisons put an equal weight on different objectives of the \ac{momdp}.
% %
% However, for the case with stochasticity in the robot's dynamic, the vectors of probabilities computed for the outcomes under the three kinds of stochastic orderings  are  different.
% }%
% \deleted{The probability of satisfying outcome $p_1$ is small because to accomplish $p_1$, the robot needs to pollinate tulips and and either orchids or daisies in exactly $12$ time steps, which is the time limit the battery can provide power to the robot, and for doing so, the robot must not encounter the bird and it should reaches those cells containing the flowers exactly when it is not raining, and that its actuators provide a high guarantee that they will move the robot to the exact cell commanded by the robot at each step.}
% \jf{the last sentence does not lead much insight into this problem.}

\section{Conclusions and Future Work}
%
In this paper, we introduced a formal language for specifying user's partially-ordered preferences over temporal goals expressed in LTL$_f$. We developed an algorithm to convert the user preference over LTL$_f$ formulas into an automaton with a preorder over the acceptance conditions. To synthesize a most preferred policy in a stochastic environment, we utilized stochastic ordering to translate a partially-ordered user's preference to a preorder over probabilistic distributions over the system trajectories. This allowed us to rank the policies based on the partially-ordered user's preference.     
Leveraging the automaton structure, we proved that computing a most-preferred policy can be reduced to finding a Pareto-optimal policy in a multi-objective \ac{mdp} augmented with the automaton states.

This work provides fundamental algorithms and principled approach for preference-based probabilistic planning with partially-ordered temporal logic objectives in stochastic systems.   
A direction for future work will be to extend the planning with preference over temporal goals that are satisfied in infinite time, for instance, recurrent properties and other more general properties in temporal logic. For robotic applications, it would be of practical interest to design a conversational-AI interface that elicits  human preferences and translating natural language specifications into the preference model, and thus facilitate human-on-the-loop planning. 



==> sections/introduction.tex <==
\added{The rise of AI and foundational models has made human-AI interactions more intuitive by enabling autonomous systems to understand human's preferences in natural language.
However, human preferences are not always expressible by a total order.
They often need to admit a \emph{partial} order because of (a) \emph{Inescapability}: agents must make decisions with limited information under time constraints, and 
(b) \emph{Incommensurability}: some comparisons, such as deciding between minimizing harm to one individual versus saving multiple lives in scenarios like the trolley problem \cite{thomson1984trolley}, lack a common basis.
While there exists a wide body of literature on preference-based planning under partial order preferences in deterministic environments (see \cite{baier2008planning} and the references within), this problem remains under-explored for probabilistic environments.
}

\deleted{With the rise of artificial intelligence and foundational models, 
robotics and other autonomous systems are now designed to understand and respond to human commands in natural language, making human-robot interactions more intuitive and user-friendly. 
However, human commands or preferences are not always expressible by a complete linear order. Preferences may need to admit a \emph{partial} order because of (a) \emph{Inescapability}: An agent has to make decisions under time limits but with partial information about preferences because, for example, it lost communication with the server; and (b) \emph{Incommensurability}: Some situations, for instance, the quality of an apple to that of banana, are fundamentally incomparable since they lack a standard basis for comparison. These situations motivate the need for 
a procedure that translates human preferences into a computational model for autonomous agents and a planner that deals with partially ordered preferences in the presence of all uncertainties in its environment
}

\replaced{We study a variant of the policy synthesis problem in a \acf{mdp} \cite{baier2004controller}, where the goal is to synthesize a policy that maximally satisfies a user preference expressed as a partial order on a set of \acf{ltlf} formulas.} 
{In this paper, we consider preference-based planning (PBP) in stochastic systems modeled as Markov decision processes (MDPs) with user preferences over temporally extended goals. Specifically, we express each temporally extended goal using a formula in Linear Temporal Logic on Finite Traces (LTL$_f$). } 

As a motivating example, consider Figure~\ref{fig:gap_garden}, which shows a garden that belongs to Bob. He grows three kinds of flowers: Tulips, daisies, and orchids. To pollinate the flowers, he uses a bee robot with limited battery. The environment is uncertain due to the presence of another agent (bird), the weather, and the robot dynamics.
%

Bob has a preference for how the robot should achieve the task of pollination. Compared to the other types, tulips have a shorter life span, so Bob considers four outcomes: % Since tulips have a shorter life span as compared to the other two kinds of flowers, Bob considers four outcomes:
% Considering the robot's battery limit and that tulips have a shorter life span when compared to the other two kinds of flowers, Bob considers four outcomes:


\begin{itemize}
    \item[($p_1$)] pollinate tulips first, then at least one other flower type; % first pollinate tulips and then pollinate at least one more kind of flowers,
    \item[($p_2$)] pollinate two types of flowers, with the first being either daisies or orchids; %pollinate at least two with first either tulips or orchids are pollinated, 
    \item[($p_3$)] pollinate only tulips; and
    \item[($p_4$)] pollinate either daisies or orchids or no flowers,
\end{itemize}
over which, his preference is shown in Figure~\ref{fig:gap_garden}b, using a preference graph, where the nodes represent the outcomes, and each directed edge \replaced{from $p_i$ to $p_j$ represents that Bob strictly prefers outcome $p_j$ over $p_i$}{
	is an improving flip [cite]
%\cite{santhanamRepresentingReasoningQualitative2016}
}. 
According to this graph, $p_1$ is the most preferred outcome, and $p_4$ is the least preferred, while $p_2$ and $p_3$ are incomparable with each other. %, are assigned to have a priority higher than $p_4$ but lower than $p_1$.
%
% These preferences are shown in Figure~\ref{fig:gap_garden}b using a preference graph, where nodes are different outcomes, and each directed edge is an improving flip \cite{santhanamRepresentingReasoningQualitative2016}. 
%
As the robot has a limited battery life and the system is stochastic, it might not achieve the most preferred outcome with probability one. %Given the robot's battery limit and the stochasticity in the system, the robot might not be able to achieve the most preferred outcome with probability one.
%
Thus, we are interested to answer the following questions: Given all the uncertainties in the environment, how to compute a robot's policy that maximally satisfies Bob's preference? 
\deleted{How to rank different policies, considering the fact that some outcomes are incomparable?} 
%\ak{The second question looks out of context. It's suitable as a part of solution approach than motivating question.} 
%  \ak{@HR: can you add a connecting statement.}


\added{The problem poses a fundamental question: \emph{Given a partial order on \ac{ltlf} formulas, how to induce a partial order on the set of policies in MDP?}
Answering this question is particularly challenging because each policy in \ac{mdp} induces a probability distribution over the set of finite paths in \ac{mdp} and each finite path in \ac{mdp} satisfies a set of \ac{ltlf} formulas. 
Consequently, comparing any two policies amounts to comparing two probability distributions over subsets of \ac{ltlf} formulas.  
}



We present a two step approach to address this challenge.
First, we introduce a computational model called \ac{pdfa}, which encodes a partial order on the subsets of \ac{ltlf} formulas as a partial order on the states of a semi-automaton, \ie, a deterministic finite automaton without final states. 


Second, we build upon the notion of stochastic orders \cite{masseyStochasticOrderingsMarkov1987} to compare policies by comparing the distributions induced by them over a family of subsets of \ac{ltlf} formulas. 
Specifically, we focus on three types of stochastic orders: strong, weak, and weak$^*$, each of which defines distinct families of subsets.
Given a partial order on a set $U$, the strong order consists of subsets $U$ that are not dominated by any element in $U$ not in the subset.
A policy is strictly preferred to another under the strong stochastic order if the probability of satisfying some of the undominated subsets in this family is strictly greater under the first policy than the second, while remaining equal for all others. 
In fact, the notion of strong stochastic order coincides widely studied concept of stochastic dominance, but is known to result in conservative outcomes \cite{masseyStochasticOrderingsMarkov1987}.

%Specifically, we consider three types of stochastic orders, namely strong, weak, and weak$^*$, that define different family of subsets.
%%
%The strong order includes those subsets of \ac{ltlf} formulas in the family that are not dominated to any formula outside the subset under the given partial order on \ac{ltlf} formulas.
%Therefore, a policy is strictly preferred to another under strong stochastic order if the cumulative distribution function of the distribution induced by the first policy assigns higher probabilities to some of these undominated subsets of \ac{ltlf} formulas, while being equal at all others.
%The strong stochastic order coincides with the well-studied notion of stochastic dominance \cite{}.
%However, strong stochastic order often leads to overly conservative results; the processes that exhibit stochastic dominance in expectation or distribution may not satisfy strong stochastic order \cite{}.

%
%, where the strong stochastic order coincides with the stochastic dominance \cite{}.
%
Weak and weak$^*$ stochastic orders offer less conservative way to compare policies. 
%A policy is considered weakly preferred to another under strong order if the cumulative distribution function of the probability distribution induced by the first policy over the set of subsets of \ac{ltlf} formulas is greater than or equal to that of the distribution induced by the second policy \cite{}.
%
%A probability distribution induced by a policy under strong order is weakly preferred to another  
%
%a distribution $X$ is weakly preferred to $Y$ if cumulative distribution of $X$ is greater than or equal to that of $Y$ for all points in the domain \cite{}.
For each \ac{ltlf} formula, the family of subsets induced by the weak stochastic order includes a subset containing all \ac{ltlf} formulas \emph{at least as good as} as the formula under given partial order on \ac{ltlf} formulas. 
Whereas, the weak$^*$ stochastic order accounts for incomparable outcomes by including a subset for each \ac{ltlf} formula containing all \ac{ltlf} formulas \emph{no worse than} the formula.
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/GapsGarden.png}
    \caption{
     \textbf{a)} Bob's Garden.
     \textbf{b)} Bob's preferences on how the bee robot should perform the task of pollinating the flowers.
    }
    \label{fig:gap_garden}
\end{figure}
%
%includes a subset of \ac{ltlf} formulas that are \emph{at least as good as}
%
%those subsets of \ac{ltlf} formulas in the family that are not dominated to any formula outside the subset under the given partial order on \ac{ltlf} formulas.
%
%the probability distribution induced by a policy under weak order indicates the likelihood of satisfying a subset of \ac{ltlf} formulas that is considered \emph{at least as good as} the subset of formulas satisfied by terminating the path at the current state.
%Similarly, under weak$^*$ order, the probability distribution indicates likelihood of satisfying a subset of \ac{ltlf} formulas that is considered \emph{no worse than} the subset of formulas satisfied by terminating the path at the current state.

The three stochastic orders satisfy a special condition: Any non-dominated policy under these stochastic order is a Pareto optimal policy in a multi-objective \ac{mdp}, which is constructed using the original \ac{mdp} and the \ac{pdfa}.
As a result, to synthesize a strategy that maximally satisfies a given preference, we solve for Pareto-optimal strategies in the corresponding multi-objective \ac{mdp}, where \emph{maximally satisfies} is interpreted under one of the three orders.


Our contributions in this paper as follows: (1) We introduce a new computational model called \emph{Preference Deterministic Finite Automaton (PDFA)}, which models a user's (possibly partially-ordered) preference  over temporally extended goals. (2) We introduce an algorithm that translates a set of partially ordered LTL$_f$ formulas, each representing a temporal goal, to a PDFA. (3) We establish a connection between the PBP in stochastic systems and the notions of stochastic orders~\cite{masseyStochasticOrderingsMarkov1987}. This connection allows us to rank policies given their induced probabilistic distribution over possible outcomes. 
%
Hence, it 
reduces probabilistic planning with partially-ordered preferences over temporal goals to computing the set of nondominated policies for a multi-objective \ac{mdp}, constructed as a product of the \ac{mdp} modeling the environment and the PDFA specifying the user preference over the temporal goals.
(4) We employ the property of weak-stochastic nondominated policies to design multiple objective functions in the product \ac{mdp} and prove that a Pareto-optimal policy in the resulting multi-objective product \ac{mdp} is weak-stochastic nondominated respecting the preference relation. Thus,  
the set of weak-stochastic nondominated policies can, then, be computed using any off-the-shelf solver that computes Pareto optimal policies.

% \jf{Here include a related work: for example you can start with, the PBP problem has been extensively investigated for deterministic planner, which [...]. However, these deterministic planners do not apply for stochastic systems for [REASONS]. ---or copy+paste the current related work and highlight the limitations. then your contribution next will be very clear what limitations are addressed.}
\subsection{Related Work}   

% %\ak{Shall we remove para titles?}
% % \jf{yes, removed}
% Preference-based planning (PBP) enables the system to decide which goals to satisfy when not all of them can be achieved \cite{hastie2010rational}. 
% Even though PBP has been studied since the early 1950's, most works on preference-based temporal planning (c.f. \cite{baier2008planning}) assume that all outcomes are pairwise comparable---that is, the preference relation is a \emph{total} order. 
% %
% This assumption is often strong and, in many cases, unrealistic \cite{aumann1962utility}. 

% {\color{red} -- This is motivation. This could be included at the beginning or removed. I'm not sure how valuable the connection to LLM methods is to automatica readers-----
% \added{Moreover, w}ith the emergence of large language models \added{and the techniques to translate} \deleted{translating} human commands into temporal logic formulas \cite{chen2023nl2tl,coslerNl2specInteractivelyTranslating2023a}, 
% it becomes natural to consider developing PBP algorithms with human preferences over temporal goals, which are commonly encountered in robotic planning problems. 
% }

% \textbf{PBP in Deterministic Environments.}
% \deleted{Setting aside natural language understanding, }
Preference-based planning (PBP) has been well-studied for deterministic systems given both total and partial preferences. See the survey by \cite{baier2008planning}.
For preferences over temporal goals in deterministic systems, several works \cite{tumova2013least,wongpiromsarn2021,rahmani2020what,rahmani2019optimal} proposed minimum-violation planning methods that decide which low-priority constraints should be violated. %in a deterministic system. 
%
\cite{amorese2023optimal} formulate and solve a two-objective optimal planning problem where one objective is to minimize the total cost of a plan, while the other aims to optimize the costs of  individual temporal goals ordered by the user preference.
%
In \cite{mehdipourSpecifyingUserPreferences2021}, authors associate weights with Boolean and temporal operators in signal temporal logic to specify the importance of satisfying the sub-formulas and priority in the timing of satisfaction. This reduces the PBP problem to that of maximizing the weighted satisfaction in deterministic dynamical systems. 
%
%\added{
For planning under this new specification language, \cite{cardona2023mixed} propose an algorithm based on mixed linear integer programming.
%}
% Robust and recovery specifications are introduced by \cite{bloem2019synthesizing} and pre-specify what behaviors are expected when the part of the system specification (\ie, the environment assumption) fails to be satisfied. 
However, the solutions to PBP  for deterministic systems cannot be applied to stochastic systems (such as  MDPs/POMDPs).
% Since a (deterministic) policy in a deterministic system results in a unique outcome, a better policy is the one that yields a better outcome. 
This is because in stochastic systems, even a deterministic policy yields a distribution over outcomes. Hence, to determine a better policy, we need comparison of distributions---a task a deterministic planner cannot do.

%  To the best of our knowledge, Li et. al \cite{} and Fu \cite{} are the only papers that study the PBP problem under a probabilistic setting. \cite{} solves the PBP problem defined over outcomes represented using Probabilistic Linear Temporal Logic by reducing it to a multi-objective model checking problem. However, they only consider the preferences representable by total orders. \ak{This restriction is relaxed in our previous work \cite{}, wherein we encode the problem of planning with partial preferences in a bounded-horizon \ac{mdp} into a Mixed Integer Linear Programming problem, which is NP-hard.} 
% In the existing solutions for probabilistic planning under temporal goals, the desired behavior of the system is specified by a temporal logic formula \cite{manna2012temporal}, and the goal is to compute a policy that either maximizes the probability of satisfying a single formula \cite{ding2011mdp,hasanbeig2019reinforcement}, or enforces the satisfaction as a constraint  \cite{Lacerda2014,wen2015correct}. 
%The PBP problem for stochastic systems has been studied recently.  
Preference-based planning for stochastic systems has been less studied until recently. In
%
\cite{Lahijanian2016}, the authors consider  to revise a given specification to improve the probability of satisfaction of the specification. They
%{proposed an
%automated specification-revision approach where the formula can be revised with a cost and the planning problem is} 
develop an \ac{mdp} planning algorithm that trades off minimizing the cost of revision and maximizing the probability of satisfying the revised formula. 
%
In
\cite{cai2021optimal}, the authors focus on planning with infeasible LTL specifications in MDPs. 
%
Their problem's objective is to synthesize a policy that, in decreasing order of importance, 1) provides a desired guarantee to satisfy the task, 2) satisfies the specifications as much as possible, and 3) minimizes the implementation cost of the plan.
%
% \cite{li2020probabilistic} solve a preference-based probabilistic planning problem by reducing it to a multi-objective model checking problem. 
%
In \cite{liProbabilisticPlanningPrioritized2023},  a fuzzy logic is introduced to capture a class of preferences over temporal goals constructed using prioritized conjunction and ordered disjunction. The authors show that these formulas can be equivalently expressed by weighted automata. They then provide a probabilistic planning algorithm that maximizes the  expected degree of satisfaction. 
However, all these works assume that the preference relation to be \emph{total}. 
%
To the best of our knowledge, only \cite{fu2021probabilistic} and \cite{kulkarni2022opportunistic} have studied probabilistic planning with incomplete preferences. 
%
Ref.~\cite{kulkarni2022opportunistic} focus on the qualitative version of the problem, synthesizing strategies that identify and exploit opportunities to improve the most preferred achievable outcome with either positive probability or probability one. This is achieved by reducing the problem to reactive synthesis \cite{manna2012temporal,baier2008principles}. In \cite{fu2021probabilistic}, the author introduced the notion of the value of preference satisfaction for planning within a pre-defined finite time duration and developed a mixed-integer linear program to maximize the satisfaction value for a subset of preference relations. In comparison, our work resorts to the notion of stochastic ordering to rank the policies in the stochastic system with respect to the partial order of temporal goals and allows the time horizon to be finite, but unbounded. 

%

%

The paper is organized as follows.
%
In Section~\ref{sec:preliminaries}, we present preliminaries and our problem definition.
%
In Section~\ref{sec:modeling_preferences}, we introduce \ac{pdfa}, and in Section~\ref{sec:pdfa}, we present our algorithm for converting a preference model of a set of LTL$_f$ formulas into a \ac{pdfa}.
%
In Section~\ref{sec:synthesis}, we present our algorithm for computing a nondominated a policy, given the \ac{pdfa} specifying the user's preference over temporal goals.
%
In Section~\ref{sec:case_study}, we present a case study and our detailed analysis.
%

\textbf{Note.} We presented a preliminary version of this paper at the 2023 IEEE International Conference 
on Robotics and Automation~\cite{rahmani2023probabilistic}. 
%
In addition to revisions made throughout the paper, we have included several new results: (1) Our preliminary version assumed the \ac{pdfa} is given by the user, but in this version we assume the user's preference is specified using a partially ordered set of LTL$_f$ formulas, and develop an algorithm to translate the partially ordered set of LTL$_f$ formulas into a \ac{pdfa}; (2) the preliminary version considered only the notion of weak-stohastic ordering for comparing policies, but in this version we added two additional notions of stochastic ordering, strong-stochastic ordering and weak$^\ast$-stochastic ordering; and (3) we extended our experiment to include results for the new additional stochastic orderings and discuss how different stochastic orders may affect the policy choices.   


==> sections/modeling_preferences.tex <==
%\subsection{Preference Modeling}
In this section, we consider the case when the user defines his preference $\langle \Sigma^\ast, \succeq \rangle$ using a ranking over temporal goals. 
%and how that preference is translated into a preference model $\langle \Sigma^\ast, \succeq \rangle$ which is a partially ordered  set of all traces generated by the MDP.
% In this section, we introduce a new combinative preference model over a (potentially infinite) set of finite words.

% Preference model. 
% \begin{definition}
% \label{def:preference-model}
% A preference model is a tuple $\langle U, \succeq \rangle$, where $U$ is a countable set of outcomes and $\succeq$ is a reflexive and transitive binary relation on $U$.
% \end{definition}


% Given $u_1, u_2 \in U$, we write $u_1 \succeq u_2$ if $u_1$ is \emph{weakly preferred to} (\ie,  is at least as good as) $u_2$; and $u_1\sim u_2$ if $u_1\succeq u_2$ and $u_2 \succeq u_1$, that is,  $u_1$ and $u_2$ are \emph{indifferent}. We write $u_1 \succ u_2$ to mean that $u_1$ is \emph{strictly preferred} to $u_2$, \ie, $u_1\succeq u_2$ and $u_2 \not\succeq u_1$.  We write $u_1 \nparallel u_2$ if $u_1$ and $u_2$ are \emph{incomparable}. Since Def.~\ref{def:preference-model} allows outcomes to be incomparable, it models \emph{incomplete} preferences \cite{bouyssou2009concepts}.


% The user specifies the temporal goals using \ac{ltlf} formulas, one formula for each goal, and then expresses their preference over these goals using a
% preference model over the set of these formulas. 
%For example, user may specify that ``visiting A and B is preferred to visiting only A.'' To this end, we consider the preference model for the agent to be $\langle \mathbb{F}, \weakpref \rangle$, where $\mathbb{F} = \{\reach{F_1}, \reach{F_2}, \ldots, \reach{F_n}\}$ is a set of reachability objectives where $F_1, \ldots, F_n$ are subsets of $S$. 

\begin{definition}
\label{def:preference-model-ltl}
%\replaced{
	An \emph{\ac{ltlf} preference model} is a preference model $\langle \Phi, \weakpref \rangle$ in which $\Phi = \{\varphi_1,\ldots, \varphi_N \}$ is a finite set of  \emph{distinct} \ac{ltlf} formulas over a set of atomic propositions $\calAP$ and $\weakpref$ is a partial order---a reflexive, transitive, and an antisymmetric---relation on $\Phi$.
	%}
% {
	% A preference model over a set of outcomes expressed in temporal logic formulas is a tuple $\langle \Phi, \weakpref \rangle$, where $\Phi = \{\varphi_1,\ldots, \varphi_N \}$ is a finite set of \emph{distinct} \ac{ltl}$_f $ formulas over the set of atomic propositions $\calAP$. 
	% }
\end{definition}
%

Two \ac{ltlf} formulas $\varphi$ and $\varphi'$ are distinct if $\mathcal{L}(\varphi) \ne \mathcal{L}(\varphi')$, where $\mathcal{L}(\varphi)$ is the language of the formula, \ie, the set of words satisfying the formula. 
%\aknote{Removed `recall' since I didn't see `distinct' LTLf defined in preliminaries?}

% \begin{remark}
% 	\ak{Comment on how a set of arbitrary \ac{ltl}$_f$ formulas can be transformed into a set of distinct \ac{ltl}$_f$ formulas.}
% \end{remark}

\begin{assumption}
\label{assume:cover}
We assume that $\bigcup_{1 \leq i \leq N} \mathcal{L}(\varphi_i) = \Sigma^\ast$, meaning that for each word $w \in \Sigma^\ast$, there
is at least one $\varphi \in \Phi$ such that $w \in \mathcal{L}(\varphi)$.
%
Note that if $\bigcup_{1 \leq i \leq N} \mathcal{L}(\varphi_i) \subset \Sigma^\ast$, then the assumption will hold by adding the formula $\varphi = \bigwedge_{1 \leq i \leq N} \neg \varphi_i$ to $\Phi$.
\end{assumption}

\begin{assumption}
\label{assume:partial-order}
The preference model $\langle \Phi, \weakpref \rangle$ is a partial order relation over $\Phi$, which means the following properties are satisfied:
\begin{itemize}
	\item Reflexive: $\varphi \weakpref \varphi$ for all $\varphi\in \Phi$.
	\item Antisymmetric: $\varphi \weakpref \varphi'$ and $\varphi'\weakpref \varphi$ implies $\varphi=\varphi'$.
	\item Transitive: $\varphi_1\weakpref  \varphi_2$ and $\varphi_2 \weakpref \varphi_3$ implies $\varphi_1\weakpref \varphi_3$.
\end{itemize}
%\aknote{shall we use $\varphi$ instead of $\varphi$?}
\end{assumption}	

\begin{remark}
%\replaced{
	Note that any preference model $\langle \Phi, \weakpref \rangle$ in which $\weakpref$ is a preorder, \ie, a partial order without the requirement of being antisymmetric, can be converted into a preference model $\langle \Phi', \weakpref' \rangle$ in which $\weakpref'$ is a partial order. 
	%}
% {Note that any preference model $\langle \Phi, \weakpref \rangle$ in which $\weakpref$ is a preorder but not a partial order, i.e. a preorder order without the requirement of being antisymmetric, can be converted into a preference model $\langle \Phi', \weakpref' \rangle$ in which $\weakpref'$ is a partial order. }
%\aknote{Assumption 2 defines partial order. Hence, I revised the statement to explain the notion of preorder in terms of partial order.}
%
The idea is to iteratively refine the preference model until the resulting model has no pair of indifferent formulas.
%
In each step, two indifferent formulas $\varphi_i$ and $\varphi_j$ are replaced by their disjunction $\varphi_i \lor \varphi_j$, after which the preference relation is altered accordingly.  
%
% Given a arbitrary preorder $\langle \Phi, \weakpref \rangle$, we can construct a partial order $\langle \Phi', \weakpref' \rangle$ by replacing every $\varphi_i, \varphi_j \in \Phi$ such that $\varphi_i \sim \varphi_j$ with their disjunction in $\Phi$ and $\weakpref$. That is, we replace $\varphi_i $ with $\varphi_i \lor \varphi_j$, $\varphi_j $ with $ \varphi_i \lor \varphi_j$ and then  construct $\Phi'$ and $\weakpref'$ after these replacements. We repeat this process until all indifferent outcomes are combined using disjunction. After this the input preorder is revised to be a partial order.
%
% \hr{I think this process is not right when the model contains at least three distinct formulas $\varphi_i, \varphi_j, \varphi_k \in \Phi$ that are indifferent, but the author probably guesses what this process means. 
	% %
	% More accurate algorithm is to partition the formulas in a way that each block contains only indifferent formulas and that for each block $B$ there is no other block $B'$ such that $B'$ contains a formula indifferent with a formula in $B$. Then create for each block $B$, a  formula $\varphi_B$ which is the disjunction of all the formulas within that block. Then, for each two distinct block $B, B'$, $\varphi_{B} \weakpref' \varphi_{B'}$ iff there are $\varphi_i \in B$ and $\varphi_j \in B'$ such that $\varphi_i \weakpref \varphi_j$. 
	% %
	% If you still want to use your process, we may mention that this process of merging two indifferent formulas should be continued until no more tuples of indifferent formulas exist.
	% }
% \ak{Yes, I missed the repeat clause. I'm okay with both procedures.}
\end{remark}

%	
%A  preference $\varphi_1 \weakpref \varphi_2$  means satisfying $\varphi_1$ is at least as good as satisfying $\varphi_2$. Specifically,  the ``at least as good as '' is formalized by
%\begin{itemize}
%	\item For any $ w_1 \models \varphi_1$ and any $w_2 \models \varphi_2$, $w_1\succeq w_2$.
%	\item There exists at least one $w_1\models \varphi_1$ and $w_2\models \varphi_2$, $w_1\succ w_2$.
%\end{itemize}
%Note that the second statement is to emphasize that some word satisfying $\varphi_1$ is strictly preferred to some word satisfying $\varphi_2$. If such a condition does not hold, then for any $ w_1 \models \varphi_1$ and any $w_2 \models \varphi_2$, $w_1\sim  w_2$---in this case, we will just use a formula $\varphi_1\lor \varphi_2$ to describe the indifference between satisfying these two formulas.
%% We assume $\varphi_1\land \varphi_2 = \falsev$. In other words, there is no word satisfying $\varphi_1$ and $\varphi_2$ simultaneously. 
%	



The model $\langle \Phi, \weakpref \rangle$ is a combinative preference model, as opposed to an exclusionary one. This is because we do not assert the exclusivity condition $ \varphi_i\land \varphi_j = \falsev$. This allows us to represent a preference such as ``Visiting A and B is preferred to visiting A,'' ($\Eventually A\land \Eventually B\weakpref \Eventually A$) where the less preferred outcome must be satisfied first in order to satisfy the more preferred outcome. In literature, it is common to study exclusionary preference models (see \cite{baier2008planning,bienvenu2011specifying} and the references within) because of their simplicity \cite{stanford2022preferences}.  
%\hr{This citation didn't show the year of the article, and so I changed the bib record of this reference in sample.bib. Please check if it looks good.}
%
However, we focus on planning with combinative preferences since they are more expressive than the exclusionary ones \cite{hansson2001structure}.  In fact, every exclusionary preference model can be transformed into a combinative one, but the opposite is not true. 

%In our case, it may be possible to transform the combinative model into an exclusionary one defined over the powerset of $\mathbb{F}$ \cite{Hansson2001}.  
%
%In literature, it is common to study exclusionary preference models (see \cite{BienvenuSpecifying,???} and the references within) because, in many cases, a combinative preference model can be transformed into an equivalent exclusionary one and vice versa \cite{Hansson2001}. However, in our case, such a transformation incurs an exponential cost (see Appendix~\ref{}). Thus, it becomes important to plan with combinative preferences. 


When a combinative preference model is interpreted over finite words, the agent needs a way to compare the sets of temporal logic objectives satisfied by two words. 
For instance, consider the preference that ``Visiting A and B is preferred to visiting A,'' and let $w_1=\emptyset \{A\}\emptyset \{B\}$ and $w_2 = \emptyset \{A\} \emptyset$ be two finite
words. 
Note that $w_1$ has both $A$ and $B$ evaluated true, each at some point in time, and $w_2 = \emptyset \{A\} \emptyset $ only has $A$ evaluated true. 
%Suppose that $w_1 = \emptyset \{A\}\emptyset \{B\} $ has  both $A$ and $B$ evaluated true at some point in time, and $w_2 = \emptyset \{A\} \emptyset $ only has $A$ evaluated true. 
Therefore, $w_1\models \varphi_1 \land \varphi_2$, whereas $w_2$ satisfies only $\varphi_2$. To determine the preference between $w_1$ and $w_2$, the agent compares the set $\{\varphi_1,\varphi_2\}$ with $\{\varphi_2\}$ to conclude that $w_1$ is preferred over $w_2$. However, suppose the given preference is that ``visiting A is preferred over visiting B,'' i.e., ($\Eventually A\weakpref \Eventually B$). Then the two words $w_1$ and $w_2$ are indifferent since both satisfy the more preferred objective $\Eventually A$.  To formalize this notion, we define the notion of most-preferred outcomes.


Given a non-empty subset $\mathbb{X} \subseteq \Phi$, let $\mathsf{MP}(\mathbb{X}) \triangleq \{\varphi \in \mathbb{X} \mid \nexists \varphi' \in \mathbb{X}: \varphi' \weakpref \varphi\}$ denote the set of most-preferred outcomes in $\mathbb{X}$.
%\jf{pay attention the use of $\strictpref$ and $\succ$.}

%For notational convenience, let $\Sigma\coloneqq 2^\calAP$. 
\begin{definition}
\label{def:mp-outcomes}
Given an \ac{ltlf} preference model $\langle \Phi, \weakpref \rangle$ and a finite word $w  \in \Sigma^\ast$, the set of most-preferred formulas satisfied by $w$ is given by $\mathsf{MP}(w) \coloneqq \mathsf{MP}(\{ \varphi \in \Phi \mid  w\models \varphi\})$. 
\end{definition}


By definition, there is no outcome included in $\mathsf{MP}(w)$ that is weakly preferred to any other outcome in $\mathsf{MP}(w)$. Thus, we have the following result.

\begin{lemma}
\label{lma:incomparable-in-MP}
For any word $w \in \Sigma^\ast$, formulas in $\mathsf{MP}(w)$ are incomparable to each other. 
\end{lemma}
%  \color{red}
% \begin{proof}
% 	By contradiction. Suppose set $\mathsf{MP}(w)$ contains two formulas $\varphi_1$ and $\varphi_2$ that are comparable. 
%     Then, either 
% 	\begin{inparaenum}[1)]
	% 		\item $\varphi_1 \strictpref \varphi_2$, or
	% 		\item $\varphi_2 \strictpref \varphi_1$, or
	%         \item $\varphi_2 \sim \varphi_1$.
	% 	\end{inparaenum} 
% 	If one of the first two cases holds, then only one of the formulas $\varphi_1$ and $\varphi_2$ is included in $\mathsf{MP}(w)$, and this a contradiction. 
%     %
%     \replaced{
	%     The third case cannot hold because we assumed $\weakpref$ is antisymmetric.}
%     {
	%     If the third case holds, then none of $\varphi_1$ and $\varphi_2$ is included in $\mathsf{MP}(w)$, which is contradiction too.
	%     }
% \end{proof}
%\color{blue}
\begin{proof}
By contradiction. Suppose that the set $\mathsf{MP}(w)$ contains two formulas $\varphi_1$ and $\varphi_2$ that are comparable. Then, since $\weakpref$ is a partial order, one of the following cases must be true:  
\begin{inparaenum}[1)]
	\item $\varphi_1 \strictpref \varphi_2$, or
	\item $\varphi_2 \strictpref \varphi_1$.
	% \item $\varphi_2 \sim \varphi_1$.
\end{inparaenum} 
Consider the first case. By definition of $\mathsf{MP}$ operator, only $\varphi_1$ is included in $\mathsf{MP}(w)$. Similarly, in second case, only $\varphi_2$ is included in $\mathsf{MP}(w)$. This is a contradiction. 
\end{proof}
%\normalcolor


Now, we formally define the interpretation of $\langle \Phi, \weakpref \rangle$ in terms of the preference relation it induces on $\Sigma^\ast$.

\begin{definition}
\label{def:preference-ltl}
An \ac{ltlf} preference model $\langle \Phi, \weakpref \rangle$ induces the preference model $\langle \Sigma^\ast, \succeq \rangle$ where for any $w_1, w_2 \in \Sigma^\ast$, 

\begin{itemize}
	\item $w_1 \succeq w_2$ if and only if  for every formula $\varphi \in \mathsf{MP}(w_1)$, there exists a formula  $\varphi'\in \mathsf{MP}(w_2)$ such that $\varphi \weakpref \varphi'$,  
	
	\item $w_1 \sim w_2$ if and only if $\mathsf{MP}(w_1) = \mathsf{MP}(w_2)$, and
	
	\item $w_1 \nparallel w_2$, otherwise.
\end{itemize}
\end{definition}

% \hr{If no formula satisfies $w_1$, then for any $w_2$, $w_1 \succeq w_2$ because $\mathsf{MP}(w_1) = \emptyset$, meaning that the first condition in the above list vacuously holds. I think this is problematic, and so I added the Assumption~\ref{assume:cover} that if every word is satisfied by at least one formula.}
% \jf{I agree. if it is fine with all we can remove this comment. }

% \deleted{Note that the first condition does not say, for any $\varphi'\in \mathsf{MP}(w_2)$, there exists $\varphi \in \mathsf{MP}(w_1)$ that $\varphi \weakpref \varphi'$.  Therefore, there can be some formula in $\mathsf{MP}(w_2)$ that is incomparable to any formula in   $\mathsf{MP}(w_1)$.}\ak{---this was internal remark.}

The following set of properties can be shown.


\begin{lemma}
Let $\langle \Sigma^\ast, \succeq \rangle$ be the preference model induced by $\langle \Phi, \weakpref \rangle$. For any $w_1, w_2\in \Sigma^\ast$, if $w_1\succeq w_2$, then   
there does not exist a pair of outcomes $\varphi \in \mathsf{MP}(w_1)$ and $\varphi' \in \mathsf{MP}(w_2)$ such that $\varphi' \weakpref \varphi$.
\end{lemma}
\begin{proof}
By contradiction.
Let $ \mathsf{MP}(w_1) = \{\varphi_1,\ldots, \varphi_m\}  $ and $\mathsf{MP}(w_2) = \{\psi_1,\ldots, \psi_t\}$. 
%
Suppose there exists $\psi \in \mathsf{MP}(w_2)$ such that $\psi \weakpref \varphi$ for some $\varphi \in \mathsf{MP}(w_1)$. 
%
Given the assumption $w_1 \succeq w_2$, by Definition~\ref{def:preference-ltl}, there exists $\psi' \in \mathsf{MP}(w_2)$ such that $\varphi \weakpref \psi'$. 
%
As a result, $\psi \weakpref \varphi \weakpref \psi'$, implying that $\psi \weakpref \psi'$. This contradicts the result in Lemma~\ref{lma:incomparable-in-MP} which imposes $\mathsf{MP}(w_2)$ to contain only incomparable formulas. 
%
Thus, the assumption that $\psi \weakpref \varphi$ is contradicted.
\end{proof} 
%\jf{There is inconsistent notation. initially you have $\varphi_i,\psi_j$ and then you have $\varphi, \varphi'$, please check.}


\begin{lemma}
If $w_1 \sim w_2$, then $\mathsf{MP}(w_1)= \mathsf{MP}(w_2)$.
\end{lemma}
%\aknote{conforming to Def. 11.}
\begin{proof}
By way of contradiction, suppose $\mathsf{MP}(w_1)\ne \mathsf{MP}(w_2)$. 
%
Without loss of generality, let $\varphi \in \mathsf{MP}(w_1) \setminus \mathsf{MP}(w_2)$. 
%
Given $w_1\succeq w_2$ and $\varphi \in \mathsf{MP}(w_1)$, there must exist a formula $\psi\in \mathsf{MP}(w_2)$ such that $\varphi \weakpref \psi$. 
%
Also, because $w_2\succeq w_1$, there exists a formula $\phi \in \mathsf{MP}(w_1)$ such that $\psi \weakpref \phi$. 
%
Due to the transitivity of $\weakpref$, $\varphi \weakpref \psi \weakpref \phi$ and thus $\varphi \weakpref \phi$ and that $\varphi, \phi \in \mathsf{MP}(w_1)$, contradicting Lemma~\ref{lma:incomparable-in-MP}. 
%
Since $\varphi$ is chosen arbitrarily, witnessing this contradiction implies that $\mathsf{MP}(w_1)= \mathsf{MP}(w_2)$.
\end{proof}

% \jf{adding one paragraph to remind the reader the difference between partial order and preorder.} \ak{See Remark 1. Would that be sufficient? }
% \hr{We can even move that Remark to the previous section where we defined "preference model", after Definition~\ref{def:model_preference}.
% We may not even have to have Definition~\ref{def:preference-model-ltl}, which defines the notion of "preference model over \ac{ltlf} formulas". We have already defined in Definition~\ref{def:model_preference} what is a "preference model". So basically the preference model $\langle \Phi, \weakpref \rangle$ iin terms of Definition~\ref{def:preference-model} is the preference model $\langle \Phi, \succeq \rangle$ where $\weakpref = \succeq$.
% We replace $\weakpref$ with $ \succeq$ in the entire paper.
% }
% \jf{I think the remark makes sense. I wonder if there is an agreement to replace $\weakpref$ by $\succeq$? I am ok with keeping these two separated.}
% \ak{Do you suggest using $\langle \Phi, \succeq \rangle$ instead of $\langle \Phi, \weakpref \rangle$ to represent preference over \ac{ltlf} and using $\langle \Sigma^*, \succeq \rangle$ for preference over words? If yes, then this is technically incorrect. $\succeq, \weakpref$ are two sets representing the binary relation that contain different elements.}

\begin{lemma}
The preference model $\langle \Sigma^\ast, \succeq \rangle$  induced by $\langle \Phi, \weakpref \rangle$ is a   preorder. 
\end{lemma}
\begin{proof}
For any $w\in \Sigma^\ast$, $w \succeq w$ because for any $\varphi\in \mathsf{MP}(w)$, $\varphi\weakpref \varphi$.
Thus, $\langle \Sigma^\ast, \succeq \rangle$ is reflexive. %because for any $w\in \Sigma^\ast$, for any $\varphi\in \mathsf{MP}(w)$, $\varphi\weakpref \varphi$. 
%Thus $w \succeq w$.
%
For the transitivity, supposing $w_1\weakpref w_2$ and $w_2\weakpref w_3$, we need to show that $w_1\weakpref w_3$. 
%
Let for each $t \in \{1, 2, 3 \}$, $\mathsf{MP}(w_t)=\{\varphi_{t, i}\mid i=1,\ldots, n_t \}$ be the most prefered formulas satisfied by $w_t$.
%
% Consider the most preferred formulas satisfied by $w_1,w_2,w_3$ respectively as 
% $\mathsf{MP}(w_1)=\{\varphi_{1,i}\mid i=1,\ldots, n_1 \}$,
% $\mathsf{MP}(w_2)=\{\varphi_{2,i}\mid i=1,\ldots, n_2 \}$, and
% $\mathsf{MP}(w_3)=\{\varphi_{3,i}\mid i=1,\ldots, n_3 \}$.
%
Given that $w_1\succeq w_2$, for any $\varphi_{1,i} \in \mathsf{MP}(w_1)$, there exists $\varphi_{2,j} \in \mathsf{MP}(w_2)$ such that $\varphi_{1,i} \weakpref \varphi_{2,j}$. 
%
Also, because $w_3\succeq w_3$, for any such $\varphi_{2, j}$, there exists $\varphi_{3, k} \in \mathsf{MP}(w_3)$
such that $\varphi_{2,j}\weakpref \varphi_{3,k}$. 
%
Using the transitivity property of $\weakpref$, $\varphi_{1, i}\weakpref \varphi_{3, k}$ holds. 
%
As a result, $w_1\succeq w_3$.
%
\end{proof}
Note that the preference relation $\langle \Sigma^\ast, \succeq \rangle$ needs not to be antisymmetric since there might exist two words $w_1\neq w_2$ such that $\mathsf{MP}(w_1) = \mathsf{MP}(w_2)$.
%
For example, with $\Phi = \{\Eventually a, \Eventually b \}$, consider two words $\emptyset \emptyset \{a\} \{b\}$ and $\emptyset \{a\} \emptyset \{b\}$.  
%
Since they both satisfy both $\Eventually a$ and $\Eventually b$, $w_1 \succeq w_2$ and $w_2 \succeq w_1$, while $w_1 \neq w_2$, showing an example where $\succeq$ is not antisymmetric.

% \todo[inline]{investigate if the pre-order is monotone or not.}
% \ak{Could you elaborate what you mean by a preorder to be a monotone?}



==> sections/pdfa.tex <==
In this section, we  introduce a novel computational model called a \acf{pdfa}, which encodes the preference model $\langle \Sigma^\ast, \succeq \rangle$ into an automaton. We present a procedure to construct a \ac{pdfa} for a given preference model $\calP = \langle \Phi, \weakpref \rangle$ and prove its correctness with respect to the interpretation in Definition~\ref{def:preference-ltl}.  


\begin{algorithm}[t]
\caption{Construction of Preference Graph}
\label{alg:pref-graph}
\begin{algorithmic}[1]
	\Function{PrefGraph}{$\langle \Phi, \weakpref \rangle, \langle Q, \Sigma, \delta, \init \rangle$}
	\State Initialize $\prefnodes = \emptyset, \prefedges = \emptyset$, $Z =\emptyset$.
	\ForAll{$(\vec{q}, \vec{q}') \in Q\times Q$} \label{line:for} \label{line:outer_loop}
	\If{$\mathsf{MP}(\vec{q})= \mathsf{MP}(\vec{q}') $}
	\State $Z= Z\cup \{(\vec{q},\vec{q}'), (\vec{q}',\vec{q})\}$
	% \State continue. \hr{If we want to avoid this 'continue', we may consider putting the following block in an 'else' block. }
	\Else
	\State Initialize $D$ as an empty set of sets.
	\ForAll{$\varphi \in \mathsf{MP}(\vec{q})$}
	\State Add $\{\varphi' \in \mathsf{MP}(\vec{q}') \mid \varphi \weakpref \varphi'\}$ to $D$.
	\EndFor
	\If {$\emptyset \notin D$}
	\State $Z \gets Z \cup \{(\vec{q}', \vec{q})\}$. \label{line:z}
	\EndIf
	\EndIf
	\EndFor
	\State $\prefnodes \gets \mathsf{getSCC}(\langle Q, Z \rangle)$ \label{line:SCC}
	\ForAll{$\prefnode, \prefnode' \in \prefnodes$} \label{line:begin_2_loop}
	\If{$\exists \vec{q}\in \prefnode, \vec{q}'\in \prefnode': (\vec{q}, \vec{q}') \in Z$}
	\State $\prefedges\gets \prefedges \cup \{ (\prefnode, \prefnode') \}$ \label{line:end_2_loop}
	\EndIf
	\EndFor  
	\State \Return $G = \langle \prefnodes, \prefedges \rangle$
	\EndFunction 
\end{algorithmic}
\end{algorithm}


\begin{definition}
\label{def:pdfa}
A \ac{pdfa} for an alphabet $\Sigma$ is a tuple $\pdfa= \langle Q, \Sigma, \delta, \init, G:=(\prefnodes, \prefedges) \rangle$
in which $Q$ is a finite set of states;
%
$\Sigma$ is the alphabet;
%
$\delta: Q \times \Sigma \rightarrow Q$ is a transition function;
%
$\init \in Q$ is the initial state; 
%
and $G=(\prefvertices, \prefedges)$ is a \emph{preference graph} in which,
$\prefvertices = \lbrace W_1, W_2, \cdots, W_m \rbrace$ is a partition of $Q$---i.e., 
$W \subseteq Q$ for each $W \in \prefvertices$, $W \cap W' = \emptyset$ for each distinct state subsets
$W, W' \in \prefvertices$, and $\bigcup_{W \in \prefvertices} W = Q$; and $\prefedges \subseteq \prefvertices \times \prefvertices$ is a set of directed edges.
%
\end{definition}  


With a slight abuse of notation, we define the extended transition function $\delta: Q \times \Sigma^\ast \rightarrow Q$ in the usual way, \ie, $\delta(q,\sigma w) = \delta(\delta(q,\sigma), w)$ for $w\in \Sigma^\ast$ and $\sigma \in \Sigma$, and $\delta(q, \epsilon)=q$.
%
Note that Definition~\ref{def:pdfa} augments 
a \ac{dfa}
%the classical deterministic finite automaton~\cite{hopcroft2001introduction} 
with the preference graph $G$, instead of a set of accepting (final) states. 
%
%

For two vertices $W, W' \in \prefvertices$, we write $W  \rightsquigarrow W'$ to denote $W'$ is \emph{reachable} from $W$.
%
By definition, each vertex $W$ of $G$ is reachable from itself. That is, $W \rightsquigarrow W$ always holds.
%
%

The \ac{pdfa} encodes a preference model $\succeq$ for $\Sigma^*=(2^\calAP)^*$ as follows. 
%
Consider two words $w, w' \in \Sigma^*$.
%
Let $W, W' \in \prefvertices$ be the two state subsets such that $\delta(q, w) \in W $ and $\delta(q, w') \in W'$ (recall that $\prefvertices$ is a partitioning of $Q$);
There are four cases: (1) if $W  = W'$, then $w \sim w'$; (2) if $W  \neq W'$ and $W' \rightsquigarrow W $, then $w \succ w'$; (3) if $W  \neq W' $ and $W \rightsquigarrow W'$, then $w' \succ w$; and (4) otherwise, $w \nparallel w'$.


For an example, see Figure~\ref{fig:pdfa}, which shows the \ac{pdfa} for the preferences $p_1$ through $p_4$ in Figure~\ref{fig:gap_garden}.
%



Next, we describe the construction of \ac{pdfa} given a preference model $\calP = \langle \Phi, \weakpref \rangle$. 
The construction involves two steps, namely, the construction of the underlying graph of \ac{pdfa} and the construction of the preference graph. 




\begin{definition}
\label{def:product-graph}
Given a preference model $\langle  \Phi, \weakpref \rangle $,
for each formula $\varphi_i \in \Phi$, let $\calA_i = \langle Q_i, \Sigma, \delta_i, \init_i, F_i\rangle$ be the   \ac{dfa} representing the language of $\varphi_i$.
% {let for each formula $\varphi_i \in \Phi$, $\calA_i = \langle Q_i, \Sigma, \delta_i, \init_i, F_i\rangle$ be the \emph{complete} \ac{dfa} representing the language of $\varphi_i$. }
%
The underlying automaton of the \ac{pdfa} representing $\langle  \Phi, \weakpref \rangle $ is the tuple, 
\[
\langle Q, \Sigma , \delta, \init \rangle,
\]
in which $Q = Q_1 \times Q_2 \times \cdots Q_n$ is the set of states in \ac{pdfa};
$\delta: Q \times \Sigma \rightarrow Q$ is a deterministic transition function where for each $\vec{q}=(q_1, q_2, \cdots, q_n) \in Q$ and $a \in \Sigma$, $\delta(\vec{q}, a) = (\delta_1(q_1, a), \delta_2(q_2, a), \cdots, \delta(q_n, a))$; and $\vec{\init} = (\init_1, \init_2, \cdots, \init_n)$ is the initial state.
\end{definition}

%
We represent each state in $Q$ as a vector $\vec{q}$ and the $i$-th component of $\vec{q}$, denoted as $\vec{q}[i]$, is the state in $Q_i$. 


%=========================================================
% DO NOT DELETE
%=========================================================
% {\color{purple}
% \textbf{Question by LCSS (R4).} This is indeed one way to define the preference graph whose nodes are formed by considering every possible subset of $\Phi$ and considering the most-preferred outcomes in that subset. The disadvantage of this method is that it results in an exponentially large preference graph. In contrast, our preference graph is polynomial in the size of $\Phi$ because the DFA corresponding to any scLTL formula can be minimized to contain exactly one final state. Hence, the product DFA of all formulas in $\Phi$ has $O(|Q_1 ||Q_2 |\ldots|Q_n |$) states. This is also the upper-bound on number of nodes in preference graph.
% }
%=========================================================


Algorithm~\ref{alg:pref-graph} describes a procedure to construct the preference graph.  It uses the following definition that slightly abuses the notation $\mathsf{MP}(\cdot)$: For each product state $\vec{q}$, we define the set \[ \mathsf{MP}(\vec{q}) = \mathsf{MP}( \left\{ \varphi_i \in \Phi  \mid \vec{q}[i] \in F_i	\right\} ).
\]
In words, $\mathsf{MP}(\vec{q}) $ is a set of most preferred formulas satisfied by any word that ends in $\vec{q}$. 


Given the preference model $\langle \Phi,\weakpref \rangle$ and the underlying automaton $\langle Q, \Sigma , \delta, \init \rangle$ of the \ac{pdfa}, lines \texttt{\ref{line:for}-\ref{line:z}} of Algorithm~\ref{alg:pref-graph} construct a set $Z$ of directed edges such that $(\vec{q}',\vec{q})\in Z$ if 
and only if for every $\varphi \in \mathsf{MP}(\vec{q})$, there exists a formula $\varphi' \in \mathsf{MP}(\vec{q}')$  such that $\varphi \weakpref \varphi'$. %(witnessed using $\mathtt{Cond}$).
%\aknote{Updated algorithm: check.}
%
%
Lines \texttt{\ref{line:SCC}-\ref{line:end_2_loop}} of Algorithm~\ref{alg:pref-graph} shows how the set $\prefnodes$ and edges $\prefedges$ of the preference graph are constructed. Using the set of directed edges $Z$, the algorithm computes first the set $\prefnodes$ as the set of strongly connected components of the graph given by state set $Q$ and edges $Z$. Then, a directed edge from an SCC $W$ to another SCC $W'$ is added if there is a state $\vec{q}\in W$ and a state $\vec{q}\in W'$ such that $(\vec{q},\vec{q'})\in Z$. In other words, the preference graph is constructed as the meta-graph of $(Q,Z)$ based on the SCCs.

In Section~\ref{sec:case_study}, we provide a detailed explanation of the construction of the PDFA for the preferences in Figure~\ref{fig:gap_garden}, implemented through our algorithm.

We next show how the \ac{pdfa} constructed using the product operation in Definition ~\ref{def:product-graph} and Algorithm ~\ref{alg:pref-graph} encodes the exact preference model $\langle \Phi, \weakpref\rangle $. 


\begin{proposition}
	\label{prop:node-property}
	Let $\prefnodes$ be the set of nodes constructed by Algorithm~\ref{alg:pref-graph}. 
	%
	For each $\vec{q} , \vec{q'} \in Q$ for which $\mathsf{MP}(\vec{q}) =  \mathsf{MP}(\vec{q}')$, it holds that $\vec{q}$ and $\vec{q}'$ are included in the same node in $\prefnodes$.
\end{proposition}
\begin{proof}
	By the construction in Line~5 of Algorithm~\ref{alg:pref-graph} and the definition of strongly connected components \cite{cormen2022introduction}.
\end{proof}



\begin{proposition}
\label{prop:edge-property}
If  $(\vec{q} , \vec{q'})\not \in Z$, then in graph $\langle Q, Z \rangle$ there is no directed path from $\vec{q}$ to $\vec{q'}$.
\end{proposition}
\begin{proof}
	For the sake of contradiction, suppose $(\vec{q},\vec{q}')\notin Z$ but  there is a directed path of length greater than $ 1$ from $\vec{q}$ to $\vec{q}'$. Let this path be $\vec{q}_0 \rightarrow \vec{q}_1 \rightarrow \cdots   \rightarrow \vec{q}_n$ where $\vec{q}_0=\vec{q}$, $\vec{q}_n=\vec{q}'$, and  $\vec{q}_1$ through $\vec{q}_{n-1}$ are intermediate states along the path.
	%
	For $i=0,\ldots, n$,  let $X_i = \mathsf{MP}(\vec{q}_i)$. By the construction, for any $\varphi \in X_{i+1}$, there exists a formula $\psi \in X_{i}$ such that $\varphi \weakpref \psi$. Applying the transitivity of the preference $\weakpref$, it holds that for any $\varphi\in X_n = \mathsf{MP}(\vec{q}')$, there exists a formula $\psi \in X_0 = \mathsf{MP}(\vec{q})$ such that $\varphi \weakpref \psi$. 
	As a result, $(\vec{q},\vec{q}')\in Z$, contradicting the assumption.
\end{proof}


\begin{proposition}
	\label{prop:partition}
	Set $\prefnodes$ constructed by Algorithm~\ref{alg:pref-graph} partitions $Q$.
\end{proposition}
\begin{proof}
	This property automatically holds due to the property of strongly connected components \cite{cormen2022introduction}.
\end{proof}


\begin{theorem}
	Let $\langle \Sigma^\ast, \succeq \rangle $ be the preference model induced by the semantics of $\langle \Phi, \weakpref \rangle $ (Definition ~\ref{def:preference-ltl}). Given the \ac{pdfa}  $\mathcal{A} = \langle  Q, \Sigma, \delta, \init, G \rangle $ constructed for the preference model $\langle  \Phi, \weakpref \rangle$ using Definition~\ref{def:product-graph} and Algorithm~\ref{alg:pref-graph}, for any $w,w'\in \Sigma^\ast$ let $W, W' \in \prefnodes$ be the nodes such that $\delta(\init, w) \in \prefnode$ and $\delta(\init, w') \in \prefnode'$, the following statements are established:
	\begin{itemize}
		\item (Case 1)  
		$ \prefnode  = \prefnode'$ if and only if
		$w'\sim  w$.
		\item (Case 2)  $\prefnode \ne \prefnode'$ and 
		$\prefnode \rightarrow \prefnode' $ if and only if $w' \succeq w $ and $w\not\sim w'$.
		
		\item (Case 3)  $\prefnode \ne \prefnode'$ and 
		$\prefnode' \rightarrow \prefnode $ if and only if $w \succeq w' $ and $w\not\sim w'$.
		
		\item (Case 4) $w\nparallel w'$, otherwise.
	\end{itemize} 
\end{theorem} 
\begin{proof}
	Let $\vec{q} = \delta(\init, w)$ and $\vec{q}' =\delta(\init, w')$.
	By construction of the function $\mathsf{MP}(\cdot)$ and the product operation in Definition~\ref{def:product-graph}, the following equation holds:
	\begin{align*}
	\mathsf{MP}(w) 
	&= \mathsf{MP}(\{\varphi_i\mid \delta_i(\init_i, w) \in F_i \}) \\
	&=  \mathsf{MP}(\{\varphi_i\mid \vec{q}[i] \in F_i \}) \\
	&=  \mathsf{MP}(\vec{q}) 
	\end{align*}

	Case 1:  ($\Rightarrow$)  If $\prefnode=\prefnode'$, then both $\vec{q}, \vec{q}'\in \prefnode$. This means that $\vec{q}\rightsquigarrow \vec{q}'$ and $\vec{q}' \rightsquigarrow \vec{q}$.  By proposition~\ref{prop:edge-property}, it is only possible that $(\vec{q},\vec{q}')\in Z$ and $(\vec{q}',\vec{q})\in Z$. $\mathsf{MP}(\vec{q}) =  \mathsf{MP}(\vec{q}')$ can be derived due to the antisymmetric property in the partial order of $\langle \Phi, \weakpref \rangle$.
	
	($\Leftarrow$)   If $w\sim w'$, then $\mathsf{MP}(\vec{q})  = \mathsf{MP}(\vec{q}')$ and therefore $\prefnode=\prefnode'$.
	
	Case 2: ($\Rightarrow$) If $\prefnode \rightarrow \prefnode'$, 
	%\replaced{
	then given the construction of the preference graph by lines~\ref{line:begin_2_loop}-\ref{line:end_2_loop} of Algorithm~\ref{alg:pref-graph}, there exist $q \in W$ and $q' \in W'$ such that $(q, q') \in Z$.
	%}
	% {then there is a path $\vec{q}_0\rightarrow \vec{q}_1\ldots \rightarrow \vec{q}_n$ with $\vec{q}_0 = \vec{q}$ and $\vec{q}_n = \vec{q}'$ due to the property of strongly connected components.} 
	%\jf{why this is related to SCC? is it a typo?}\hr{Fixed it.} \deleted{As a result, $(\vec{q}, \vec{q}' )\in Z$ due to Proposition~\ref{prop:edge-property}.} 
	Therefore, by construction in Algorithm~\ref{alg:pref-graph}, for any $\varphi' \in \mathsf{MP}(\vec{q}')$, there is a $\varphi \in \mathsf{MP}(\vec{q})$ such that $\varphi'\weakpref \varphi$. Then, by Def.~\ref{def:preference-ltl}, $w' \succeq w$.
	
	($\Leftarrow$) If $w'\succeq w$, then $(\vec{q},\vec{q}')\in Z$. Because $W \ne W'$, then there is no path from $\vec{q}' $ to $\vec{q}$. As a result, it is not the case that $w   \succeq w'$. Thus, $w\not\sim w'$.  
	
	Case 3: proof similar to the proof of Case 2.
	
	Case 4 is a direct consequence from Cases 1, 2 and 3.
	%\end{proof}
	
	Using the computational model \ac{pdfa}, we can directly compute the set $\{w\}^\uparrow$ for any $w\in \Sigma^\ast$.
\end{proof}

\begin{lemma}
\label{lem:wUp}
For each word $w\in \Sigma^\ast$, if $\delta(\init, w)\in \prefnode$ for some $\prefnode\in \prefnodes$, then 
% \begin{itemize}
%\item 	
the upper closure of $w$ is 
\begin{align*} 
	%\{ w\}^\uparrow =\{w' \in \Sigma^\ast \mid \delta(q_0,w') = \delta(q_0, w)\} \\
	\{ w\}^\uparrow = \{w' \in \Sigma^\ast \mid \exists \prefnode' \in \prefnodes,\\ \delta(\init, w')  \in \prefnode' \text{ and } \prefnode \rightsquigarrow \prefnode'\},
\end{align*}
and the lower closure of $w$ is 
\begin{align*} 
	%\{ w\}^\uparrow =\{w' \in \Sigma^\ast \mid \delta(q_0,w') = \delta(q_0, w)\} \\
	\{ w\}^\downarrow = \{w' \in \Sigma^\ast \mid \exists \prefnode' \in \prefnodes,\\ \delta(\init, w')  \in \prefnodes' \text{ and } \prefnode' \rightsquigarrow \prefnode\}
\end{align*}
%\end{itemize}
%
\end{lemma}
The lemma directly follows from the transition function in $\pdfa$ and the transitivity property of the preference relation and thus 
the proof is omitted. 

\begin{example}
	Consider three \ac{ltlf} formulas $\varphi_1 = \Eventually a$, $\varphi_2 = \Eventually b$, and $\varphi_3 = \neg \Eventually a \wedge \neg \Eventually b$. 
	%
	Also, assume 
	%$\varphi_1 \strictpref \varphi_2 \strictpref \varphi_3$,
	$\varphi_1 \strictpref \varphi_2$, $\varphi_1 \strictpref \varphi_3$, and $\varphi_2 \nparallel \varphi_3$.
	The left column of Figure~\ref{fig:pdfa_constrcution} shows for each of the three LTL$_f$ formula, a DFA that encodes that formula.
	%
	The column in right shows the \ac{pdfa} our algorithm constructs for these three formulas and the associated user preferences.
	%
	In this \ac{pdfa}, we have written in blue for each state $x$, $\outcomes(x)$, the set of formulas satisfied when the word ends at state $x$.
	%
	For each state $x$, we have also written in red, $\mathsf{MP}(x)$---the most preferred formulas among those formulas in $\outcomes(x)$.
	%
	Accordingly,
	$\outcomes(qpr) = \{ \varphi_3 \}$, $\outcomes(q'pr')=\{\varphi_1 \}$, $\outcomes(qp'r')=\{\varphi_2\}$, and
	$\outcomes(q'p'r')=\{\varphi_1, \varphi_2\}$.
	%
	Also, $\mathsf{MP}(qpr)=\{\varphi_3 \}$, $\mathsf{MP}(q'pr')=\{\varphi_1 \}$, $\mathsf{MP}(qp'r')=\{\varphi_2 \}$, and $\mathsf{MP}(q'p'r')=\{\varphi_1\}$.
	%
	Note that because $\varphi_1 \strictpref  \varphi_2$, $\mathsf{MP}(q'p'r') = \mathsf{MP}(\{\varphi_1, \varphi_2\}) = \{\varphi_1 \}$.
	%
	Given that $\mathsf{MP}(q'p'r')=\mathsf{MP}(q'pr')$, states $q'p'r'$ and $q'pr'$ belong to the same vertex in the preference graph.
\end{example}

\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/pdfa_construction2.png}
\caption{
	PDFA for the example in Figure~\ref{fig:gap_garden}. 
	%
	\textbf{Left)} Three DFAs for three LTL$_f$ formulas $\varphi_1$, $\varphi_2$, and $\varphi_3$, for which the user preference is: $\varphi_1 \strictpref \varphi_2$,  
	$\varphi_1 \strictpref \varphi_3$, $\varphi_2 \nparallel \varphi_3$.
	%
	\textbf{Right)} The \ac{pdfa} constructed by our algorithm for the LTL$_f$ formulas and the preference over them. The output of each state---the set of formulas that satisfies every string that ends at that state---is shown in blue and the most preferred formulas for each state is shown in red.
	%
}
\label{fig:pdfa_constrcution}
\end{figure}


==> sections/preliminaries.tex <==
\textbf{Notations}: The set of all finite words over a finite alphabet $\Sigma$ is denoted $\Sigma^\ast$. 
%
The empty string, $\Sigma^0$, is denoted as $\epsilon$. 
%
%Given a finite set $X$, we use $\dist(X)$ to denote the set of all probability distributions over $X$.
We denote the set of all probability distributions over a finite set $X$ by $\dist(X)$.
%
Given a distribution $\mathbf{d}\in \dist(X)$, the probability of an outcome $x\in X$ is denoted $\mathbf{d}(x)$. %


\subsection{The System and its Policy}
%

We model the system using a variant of \ac{mdp}.

%
\begin{definition}[Terminating Labeled MDP]
\label{def:labeled_mdp}
A \ac{tlmdp}, or a terminating MDP for short, is a tuple 
$$M = \langle S, A:=\bigcup_{s \in S} A_s, \mathbf{P}, s_0, s_\bot, \calAP, L \rangle,$$ \replaced{where}{in which} 
$S$ is a finite set of states;
%
$A$ is a finite set of actions, where for each state $s \in S$, $A_s$ is the set of available actions at $s$;
%
$\mathbf{P}: S \times A   \rightarrow \dist(S)$ is the probabilistic transition  function, where for each $s, s' \in S$ and $a \in A$, $\mathbf{P}(s, a, s')$ is the probability that the MDP transitions to $s'$ after taking action $a$ at $s$; %. if $a \in A_s$, and otherwise, $\Sigma_{s' \in S}\mathbf{P}(s, a, s') = 0$;
%
$s_0 \in S$ is the initial state;
%
$s_\bot \in S$ is the \emph{termination state}, which is a unique \emph{sink} state and $A_{s_\bot} = \emptyset$; %, to which the termination action reaches, that is, for each $s\in S$, if $a_\bot \in A_s$, then $\mathbf{P}(s,a_\bot, s_\bot)=1$; % where for each state $s\in S$, if $a \in A_s$, then $\mathbf{P}(s, a, s') = 1$;
%
$\calAP$ is a finite set of atomic propositions; and
%
$L: S \rightarrow 2^{\calAP} \cup \{\epsilon\}$ is a labeling function that assigns to each state $s\in S \setminus \{s_\bot\}$, the set of atomic propositions $L(s) \subseteq \calAP $ that hold in $s$. 
Only the terminating state is labeled the empty string, i.e., $L(s)=\epsilon$ if and only if $s=s_\bot$.%, which is the empty string. %a unique symbol for the ending of a string.
\end{definition}
%


Though this definition assumes a single sink state, we do not lose generality, as one can always convert an MDP with multiple sink state into an equivalent MDP with a single sink state by  keeping only a single sink state and redirecting all the transitions to other sink states to that sink state. 
%

The robot's interaction with the environment in a finite number $k$  of steps produces an \emph{execution} $\varrho = s_0 a_0 s_1 a_1 \cdots s_{k-1} a_{k-1} s_{k}$, where $s_0$ is the initial state and at each step $0 \leq i \leq k$, the system is at state $s_i$, the robot performs $a_i \in A_{s_i}$, and then the system transitions to state $s_{i+1}$, picked randomly based on  the distribution $\mathbf{P}(\cdot \mid s_i, a_i) $.
% \aknote{$k$ steps would require the last $\varrho$ index to be $k-1$. In this case, update $0 \leq i < k-1$ since you later reference $i \mapsto i + 1$.}
% \hr{At each step the robot does an action. I mean the number of steps is the number of actions the robot does. The index of the last action is $k-1$, and so the number of actions the robot does is $k$.}
%
This execution produces a \emph{path} defined as $\rho=s_0 s_1 \cdots s_k \in S^*$, %\aknote{Since the MDP is initialized ($s_0$ is defined), wouldn't it be better to say that an execution belongs to $S^+$?} not necessarily. S^+ is a subset of S^ast.
and the \emph{trace} of this path is defined as the finite word $\trace(\rho)=L(s_0) L(s_1) L(s_2) \cdots L(s_k)  \in (2^\calAP)^*$.
%
%Execution $\rho$ is called \emph{terminating} if $s_{k} = s_\bot$.
%
Path $\rho$ is called \emph{terminating} if $s_k = s_\bot$.
%
The set of all terminating paths in $M$ is denoted $\Paths_{\bot}(M)$.
%
A policy for $M$ is a function $\pi: \mathscr{D} \rightarrow \mathscr{C}$ with $\mathscr{D} \in \{S, S^*\}$ and $\mathscr{C} \in \{A, \dist(A)\}$, and it is called \emph{memoryless} if $\mathscr{D}=S$; \emph{finite-memory} if $\mathscr{D}=S^*$; \emph{deterministic} if $\mathscr{C}=A$, and \emph{randomized} if $\mathscr{C}=\dist(A)$.

%
In a terminating \ac{mdp}, a policy is \emph{proper} if it guarantees that the termination state $s_\bot$ will be reached with probability one \cite{bertsekas1991analysis}. 	
%
The set of all randomized, finite-memory, proper polices for $M$ is denoted $\Pi_{prop}^M$. %We  are  only interested in  finite traces for which a preference relation is defined. Thus, we only consider proper policies.
%
%
%\begin{assumption}
%all the policies for the MDP are proper.
% \end{assumption}
In this paper, we consider only the \ac{tlmdp}s for which all the policies are proper. In other words, the system always terminates after a finite time. This restriction is due to that (1) 
many applications require the robot to finish its execution in a finite time, and 2) the preference specification, defined next, is restricted to a partially ordered set of finite traces. 
%

\subsection{Specifying the Temporal Goals}
%
The temporal goals in the MDP are specified formally using the following language.

\begin{definition}[Syntax of \ac{ltlf}  \cite{de2013linear}]
Given a finite set $\calAP$ of atomic propositions, a formula in \ac{ltlf} over $\calAP$ is generated by the following grammar:
\[    
\varphi \coloneqq   p \mid \neg \varphi \mid \varphi  \land \varphi  \mid \Next \varphi \mid \varphi  \until \varphi,
\]
where $p \in \calAP$ is an atomic proposition, $\neg$ and $\land$ are the standard Boolean operators negation and conjunction, respectively, and $\Next$ and $\until$ are temporal operators ``Next'' and ``Until'', respectively. 

\end{definition}
The temporal operators are interpreted over sequences of time instants. 
%
The formula $\Next \varphi$ means at the next time instant, $\varphi$ holds true. Formula $\varphi_1 \until \varphi_2$ holds true at the current time instant if there exists a future time instant at which $\varphi_2$ holds true and for all time instants from the current time until that future time, $\varphi_1$ holds true.
%
%\replaced{
An additional temporal operator ``Eventually'' ($\Eventually$) is defined as $\Eventually \varphi := \truev \until \varphi$. 
%}
%{An additional temporal operators ``Eventually'' ($\Eventually$) is define used $\land$ as $\Eventually \varphi := \truev \until \varphi$.}
%
Formula $\Eventually \varphi$ means there exists a future time instant at which $\varphi$ holds true.
%
The dual of Eventually operator is the ``Always'' ($\Always$). It is defined as $\Always \varphi := \neg \Eventually \neg \varphi$. 
%
Formula $\Always \varphi$ means $\varphi$ holds true at the current instant and all future instants. 
%
For formal semantics of \ac{ltlf}, see~\cite{de2013linear}.
%

\begin{example} \label{ex:ltlf-goals}
For the example in Figure~\ref{fig:gap_garden}, we set $\calAP = \{o, d, t \}$, in which
$o$ means orchids are   pollinated, $d$ means daisies are   pollinated, and $t$ means tulips are   pollinated. 
The temporal goals $p_1$ through $p_4$ in the example in that figure are expressed using the following \ac{ltlf} formulas:
%\hr{Add descriptions of the APs.}
% \begin{itemize}
%     \item $p_1$: \emph{pollinate tulips first, then at least one out of daisies and orchids}, $(\neg d \wedge \neg o) \until (t \wedge \Next \Eventually ( d \vee o))$;
%     \item $p_2$: \emph{pollinate two types of flowers, with the first being either daisies or orchids}, $\neg t \until ((o \wedge \Next \Eventually (d \vee t)) \vee (d \wedge \Next \Eventually ( o \vee  t)) )$;
%     \item $p_3$: \emph{pollinate only tulips}, $(\neg d \wedge \neg o) \until (t \wedge \Always (\neg d \wedge \neg o))$; and
%     %\item $p_4$: $\neg \Eventually ( t \wedge  o \wedge  d) \vee (\neg \Eventually (t \vee d) \wedge \Eventually o) \vee (\neg \Eventually (o \vee t) \wedge \Eventually d)$
%     %\item $p_4$: $ \Always \neg ( t \vee  o \vee  d) \vee (\Always \neg (t \vee d) \wedge \Eventually o) \vee (\Always \neg (o \vee t) \wedge \Eventually d)$
%     \item $p_4$: \emph{pollinate either daisies or orchids or no flowers}, $\Always(\neg d \land \neg o \land \neg t) \lor (\Eventually o \land \Always(\neg d \land \neg t)) \lor \\ (\Eventually d \land \Always(\neg o \land \neg t))$.
%     %\aknote{It is customary to write with negations in front of atoms instead of temporal operators: $\Always(\neg d \land \neg o \land \neg t) \lor (\Eventually o \land \Always(\neg d \land \neg t)) \lor (\Eventually d \land \Always(\neg o \land \neg t))$}
% \end{itemize}
%
%\aknote{Consider including English statements here. Otherwise, readers will have to keep flipping pages to compare.}
\begin{itemize}
\item[($p_1$)] pollinate tulips first, then at least one out of daisies and orchids; % first pollinate tulips and then pollinate at least one more kind of flowers,
\begin{align*}
(\neg d \wedge \neg o) \until (t \wedge \Next \Eventually ( d \vee o)),
\end{align*}
%
\item[($p_2$)] pollinate two types of flowers, with the first being either daisies or orchids; %pollinate at least two with first either tulips or orchids are pollinated, 
\begin{align*}
\neg t \until ((o \wedge \Next \Eventually (d \vee t)) \vee (d \wedge \Next \Eventually ( o \vee  t)) ),
\end{align*}
%
\item[($p_3$)] pollinate only tulips;
\begin{align*}
(\neg d \wedge \neg o) \until (t \wedge \Always (\neg d \wedge \neg o)), \deleted{\text{and}}
\end{align*}
%
\item[($p_4$)] pollinate either daisies or orchids or no flowers;
\begin{align*}
\Always(\neg d \land \neg o \land \neg t) &\lor (\Eventually o \land \Always(\neg d \land \neg t)) \\ &\lor (\Eventually d \land \Always(\neg o \land \neg t)).
\end{align*}
\end{itemize}

\end{example}
% \aknote{LTLf of p4 does not agree with p4 in English on previous page.}
% \jf{is this addressed?}
% \ak{yes.}

%\replaced{
Given an \ac{ltlf} formula $\varphi$, the words over the alphabet $2^\calAP$ that satisfy $\varphi$, constitute the language of $\varphi$, denoted by $\lang(\varphi)$. 
% }
% {Given an \ac{ltlf} formula $\varphi$, the words over the alphabet $\Sigma := 2^\calAP$ that satisfy $\varphi$ constitutes the language of $\varphi$, which is denoted $\lang(\varphi)$. }
%
%\deleted{
In the following context, we assume $\Sigma \coloneqq 2^\calAP$.
%}
%
%\deleted{We denote by $\Sigma^\ast$, the set of all finite words over $\Sigma$.} \ak{Included in notation.}
% %

% \added{
% \begin{remark}
%     In dealing with \ac{ltlf} formulas without considering the underlying system, it is assumed that $\Sigma \coloneqq 2^\calAP$.
%     %
%     Given that we are only interested in trajectories generated by the MDP $M$, we interpret \ac{ltlf} over an alphabet whose letters are only those that are used for labeling the states of $M$, i.e.,
%     $\Sigma \coloneqq \Biogcup_{s \in S} L(s)$. 
%     %
%     This usually leads to having a smaller alphabet, which in turn, results in having smaller automata using which a preferred policy is synthesized. 
% \end{remark}
% % }
% % \jf{this remark is not needed. please justify why we need it?}
% \hr{I added justification. It usually leads to having a smaller alphabet and automata.}


The language of \ac{ltlf} formula $\varphi$ can be represented by the set of words accepted by a finite automaton defined as follows:
\begin{definition}[Deterministic Finite Automaton]
A \ac{dfa} is a tuple $\calA = \langle Q, \Sigma, \delta, q_0, F \rangle$ with a finite set of states $Q$,
a finite alphabet $\Sigma$, a deterministic transition function $\delta: Q \times \Sigma \rightarrow Q$,
an initial state $q_0\in Q$, and a set of accepting (final) states $F\subseteq Q$.  For each state $q \in Q$ and letter 
$\sigma \in \Sigma$,  $\delta(q,\sigma)=q'$ is the state reached upon reading input $\sigma$ from state $q$.
\end{definition}

%
Slightly abusing the notation, we define the extended transition function $\delta: Q \times \Sigma^* \rightarrow Q$ in the usual manner: 
$\delta(q,\sigma w)=\delta( \delta(q,\sigma),w )$ for a given $\sigma\in \Sigma$ and $w\in \Sigma^\ast$, and $\delta(q, \epsilon) = q$.
%
A word $w \in \Sigma^\ast$ is \emph{accepted} by the DFA if and only if $\delta(q, w)\in F$. 
%
The language of $\calA$, denoted $\lang(\calA)$, is set the of all words accepted by the DFA, i.e., $\lang(\calA) = \{w \in \Sigma^* \mid \delta(q, w)\in F \}$.
%

For each \ac{ltlf} formula $\varphi$, there exists a DFA $\calA_\varphi$ such that $\lang(\varphi) = \lang(\calA_\varphi)$.
%
Therefore, we can encode each \ac{ltlf} formula using a DFA 
\cite{de2013linear}.
%The \ac{dfa} $\calA_\varphi$ accepts the exact set of words satisfying $\varphi$ given the semantics of \ac{ltlf}. 



\subsection{Rank the Policies}
%

We introduce a computational model that captures the user's preference over different temporal goals. %\deleted{the robot can achieve in the environment.}
%
\begin{definition}
\label{def:model_preference}
%
A preference model is a tuple $\langle U, \succeq \rangle$ where $U$ is a countable set of outcomes and $\succeq$ is \emph{preorder}--a reflexive and transitive binary relation--on $U$.
\end{definition}
%We simply use  $\succeq$ for $\succeq^U$ if its meaning is clear from the context.
Given $u_1, u_2 \in U$, we write $u_1 \succeq u_2$ if $u_1$ is \emph{weakly preferred to} (\ie,  is at least as good as) $u_2$; and $u_1\sim u_2$ if $u_1\succeq u_2$ and $u_2\succeq u_1$,
that is,  $u_1$ and $u_2$ are \emph{indifferent}.
We write
$u_1 \succ u_2$ to mean that $u_1$ is \emph{strictly preferred} to $u_2$, \ie, $u_1\succeq u_2$ and $u_1\not \sim u_2$.  We write
$u_1 \nparallel u_2$ if $u_1$ and $u_2$ are \emph{incomparable}.
%

\begin{definition}
Given a preference model $\langle U, \succeq \rangle$,
let $X$ be  a subset of   $U$, the \emph{upper closure of $X$ }is defined by 
\[
X^\uparrow = \{y \in U\mid y \succeq x \text{ for some }x\in X \}, \text{ and }
\] 
the \emph{lower closure of $X$ }is defined by
\[
X^\downarrow = \{y \in U \mid y \preceq x  \text{ for some }x\in X \}.
\] 
% 
A set $X$ is called an \emph{increasing set} if $X = X^\uparrow$.
\end{definition}	

%\jf{I introduce the name "upper closure" and "lower closure" for these two sets. see \url{https://en.wikipedia.org/wiki/Upper_set}}



In \cite{masseyStochasticOrderingsMarkov1987}, three different stochastic orderings are introduced, called \emph{strong}, \emph{weak}, and \emph{weak$^*$} orderings. The three stochastic orderings differ in how they determine a \emph{family of subsets} of $U$. 
%

\begin{definition}\cite{masseyStochasticOrderingsMarkov1987}
Let $\mathfrak{E}_{st}(U)$, $\mathfrak{E}_{wk}(U)$, and $\mathfrak{E}_{wk*}(U)$ denote the strong, weak, and weak* orderings, respectively. 
It is defined that
\begin{align*}
\mathfrak{E}_{st}(U) &= \{\text{ all increasing sets in $2^U$} \}, \\
\mathfrak{E}_{wk}(U) &= \{\{x\}^\uparrow \mid x\in U \} \cup \{U, \emptyset\}, \\
\mathfrak{E}_{wk*}(U) &= \{E\setminus \{x\}^\downarrow \mid x\in U \} \cup \{U, \emptyset\}.
\end{align*}
\end{definition}
% 
These stochastic orderings allow us to rank probability measures defined over $U$ according to the partially ordered set $U$.
%
Let $\mathfrak{E}(U)$ be \emph{a family of subsets} of $U$ that includes $U$ itself and the empty set $\emptyset$. That is, $\mathfrak{E} \in \{\mathfrak{E}_{st}, \mathfrak{E}_{wk}, \mathfrak{E}_{wk*}\}$. 	
%

Let $P_1$ and $P_2$ be two probability measures on $U$. We say $P_2$ stochastic dominates $P_1$, denote $P_2\ge_{\mathfrak{E}}P_1$  
whenever $P_2(X) \ge_{\mathfrak{E}} P_1(X)$ for all subsets $X\in \mathfrak{E}(U)$.
It is proven that if the partial order $U$ is a total order, then the three stochastic orderings $\mathfrak{E}_{st}(U)$, $\mathfrak{E}_{wk}(U)$, and $\mathfrak{E}_{wk*}(U)$  are equivalent (see Proposition~2.5 of \cite{masseyStochasticOrderingsMarkov1987}). 
However, for a partial order, the three stochastic orderings may differ.
%\aknote{The above changes are to maintain consistency of notation used in Ex. 2, DEf. 7...}
%
% \jf{Is the following example copied from Massey's paper, if so, please remove it and add a reference only.} \ak{I think this example is important/instructional for the reader to build intuition. We could reference it and keep it if space is not a concern.}
% \hr{I think this example is not copied from Massey's paper. This example was in the initial draft and I changed the numbers and the probability distributions. I checked Massey's paper and it does not have this example.}

% \jf{ok. \replaced{Let us}{Let's} keep this example}
To illustrate, consider the following example.
%
\begin{example}
Let $U = \{a,b,c,d\}$ and  $\succeq = \{(a, b), (b, d), $ $(c, d), (a, c), (a, d) \} \cup I_U$, where $I_U$ is the identity relation on $U$ and that $(x,y)\in \succeq$ if and only if $x\succeq y$.
%
Also, consider probability measures $P_1$, $P_2$, and $P_3$ where $P_1(a)=0.5, P_1(b)=0.3, P_1(c)=0.2$, $P_2(b) = 0.5, P_2(c) = 0.3, P_2(d) = 0.2$, and $P_3(a) = 0.3, P_3(b) = 0.2, P_3(d) = 0.5$.   
%

We have
\[
\mathfrak{E}_{st}(U) = \{ \{a\}, \{a,b\}, \{a,c\}, \{a, b, c \}, \{a,b,c,d\}, \emptyset\}.
\]
%
Accordingly, 
\begin{align*}
[P_1[X]]_{X\in	\mathfrak{E}_{st}(U) } &= [0.5, 0.8, 0.7, 1, 1, 0], \\
[P_2[X]]_{X\in	\mathfrak{E}_{st}(U) } &= [0, 0.5, 0.3, 1, 1, 0],  \\ 
[P_3[X]]_{X\in 	\mathfrak{E}_{st}(U) }   &= [0.3, 0.5, 0.3, 0.5, 1, 0].
\end{align*}
%
\replaced{Since}{Therefore}, $P_1 >_{\mathfrak{E}_{st}} P_2$, $P_1 >_{\mathfrak{E}_{st}} P_3$, \replaced{neither }{. None of} $P_2$ \replaced{nor}{and} $P_3$ strong-stochastic dominates the other one.

Also, we have
\[
\mathfrak{E}_{wk}(U) = \{ \{a\}, \{a,b\}, \{a,c\}, \{a,b,c,d\}, \emptyset\}.
\]
%
%
%
Accordingly, 
\begin{align*}
[P_1[X]]_{X\in	\mathfrak{E}_{wk}(U) } &= [0.5, 0.8, 0.7, 1, 0],
\\
[P_2[X]]_{X\in	\mathfrak{E}_{wk}(U) } &= [0, 0.5, 0.3, 1, 0], \text{and}
\\
[P_3[X]]_{X\in 	\mathfrak{E}_{wk}(U) }   &= [0.3, 0.5, 0.3, 1, 0].
\end{align*}
%
Thus, $P_1 >_{\mathfrak{E}_{wk}} P_2$, $P_1 >_{\mathfrak{E}_{wk}} P_3$, and $P_3 >_{\mathfrak{E}_{wk}} P_2$.
%

Also, we have
\[
\mathfrak{E}_{wk*}(U) = \{ \{a,b\}, \{a,c\}, \{a, b, c \}, \{a,b,c,d\}, \emptyset\}.
\]
%
%
%
Accordingly, 
\begin{align*}
[P_1[X]]_{X\in	\mathfrak{E}_{wk*}(U) } &= [0.8, 0.7, 1, 1, 0],
\\
[P_2[X]]_{X\in	\mathfrak{E}_{wk*}(U) } &= [0.5, 0.3, 0.8, 1, 0], \text{and}
\\
[P_3[X]]_{X\in 	\mathfrak{E}_{wk*}(U) }  &= [0.5, 0.3, 0.5, 1, 0].
\end{align*}
%
Thus, $P_1 >_{\mathfrak{E}_{wk*}} P_2$, $P_1 >_{\mathfrak{E}_{wk*}} P_3$, and $P_2 >_{\mathfrak{E}_{wk*}} P_3$.
%
\end{example}
%
In our context, because we are interested in sequential decision-making and planning problems with a finite time termination, the set $U$ is selected to be $\Sigma^\ast$, or the set of finite traces generated by the system and its labeling function.
%
%In this context, the user preference over temporal goals is a preference model for $U=\Sigma^*$ where $\Sigma= 2^\calAP$. 
Based on the ranking of probability measures induced by each one of the stochastic orderings for $\Sigma^\ast$, we can rank the proper policies $\Pi^M_{prop}$ in the \ac{tlmdp}.
%---the set of all possible \emph{finite} traces over $\calAP$. 

Specifically, note that a proper policy $\pi: S^\ast \rightarrow \dist(A)$ produces a distribution %$\mathbf{d}^\pi \in \dist(\Paths_{\bot}(M))$
over the set of all terminating paths in the MDP $M$ such that for each terminating path $\rho \in \Paths_{\bot}(M)$,
%$\mathbf{d}^\pi(\rho)$
$\Pr^\pi(\rho)$
is the probability of generating $\rho$ when the robot uses policy $\pi$.
%
Each terminating path $\rho$ is mapped to a single word in $\Sigma^*$, namely $\trace(\rho) = L(s_0) L(s_1) \ldots$, 
%
and therefore, $\pi$ yields a distribution %$\mathbf{e}^\pi \in \dist((2^\calAP)^*)$ 
over the set of all finite words over $\Sigma$
such that for each word $w \in \Sigma^\ast$, $\Pr^\pi(w)$ is the probability that 
$\pi$ produces $w$. Formally,
\[
\Pr^\pi(w) = \sum_{\rho \in \Paths_{\bot}(M): L(\rho)=w} \Pr^\pi(\rho).
\]
%
Additionally, for a subset $X \subseteq \Sigma^*$, $\Pr^\pi(X)$ is the probability of the words  generated by $\pi$ to be within $X$. Formally,
\[
\Pr^\pi(X) = \sum_{w \in X} \Pr^\pi(w).
\] 

% 		To compare two polices, we need to compare those distributions they yield on $(2^\calAP)^\ast$,
% 		and for doing so, we resort to the idea of
% 		stochastic ordering~\cite{kamaeStochasticInequalitiesPartially1977, masseyStochasticOrderingsMarkov1987}.
% 		%

% Let $U$ be a countable space ordered by a partial order $\succeq \subseteq U\times U$. $(x,y)\in \succeq$ means $x\succeq y$, \ie, $x$ is preferred to $y$.
% 	    %

% 	In this context, we let the partially ordered set be $U=(2^\calAP)^\ast$ given
% the partial order defined by the preference model $\succeq$.
% %
% For simplicity, \replaced{Let us}{Let's} from now on $\Sigma \triangleq 2^\calAP$.

%\ac{dfa}.
%
%	Given a word $w \in \Sigma^*$, we use $F_w$ to denote the state subset $F \in \mathbb{F}$ such that 
%	$\delta(q_0, w) \in F$. 

%
%   We use the notion of weak-stochasticity to compare policies.
%
% \begin{definition}
% \label{def:weak_dominating_policies}
%          Given two proper policies $\pi_1,\pi_2$ in the terminating labeled \ac{mdp} $M$, $\pi_1$ \emph{weak-stochastic dominates} $\pi_2$, denoted $\pi_1 >_{\mathfrak{E}_{wk}} \pi_2$, if and only if for each $w \in \Sigma^\ast$, it holds$
%          that $\Pr^{\pi_1}(X_w) \ge \Pr^{\pi_1}(X_w)$ where   $X_w = \{\rho \in S^\ast \mid L(\rho)\in \{w\}^\uparrow \}$.
% \end{definition}
% Note that $\Pr^{\pi_1}(\Sigma^\ast) = \Pr^{\pi_2}(\Sigma^\ast)=1$ and $\Pr^{\pi_1}(\emptyset) = \Pr^{\pi_2}(\emptyset)=0$. 
%
%
\begin{definition}
\label{def:weak_dominating_policies}
Let $\mathfrak{E} \in \{\mathfrak{E}_{st}, \mathfrak{E}_{wk}, \mathfrak{E}_{wk*}\}$ be a stochastic ordering and $\langle U \coloneqq \Sigma^\ast, \succeq\rangle$ be a preference model.
Given two proper policies $\pi$ and $\pi'$ for the terminating labeled \ac{mdp} $M$, $\pi$ \emph{$\mathfrak{E}$-stochastic dominates} $\pi'$, denoted $\pi >_{\mathfrak{E}} \pi'$, if for each subset $X \in \mathfrak{E}(U)$, it holds
that $\Pr^{\pi}(X) \ge \Pr^{\pi'}(X)$, and there exists a subset $Y \in \mathfrak{E}(U)$ such that
$\Pr^{\pi}(Y) > \Pr^{\pi'}(Y)$.
\end{definition}


%Intuitively, $\pi_1$ weak-stochastic dominates $\pi_2$ if the $\pi_1$-induced probability measure assigns a higher probability to at least one subset in $\mathfrak{E}_{wk}(\Sigma^\ast)$ and for the other subsets, either the two probability measures induced by $\pi_1$ and $\pi_2$ have the same probabilities
%

This definition is used to introduce the following notion.
%\begin{definition}[Weak-stochastic nondominated policy]
\begin{definition}
\label{def:sto_dominance}
A proper policy $\pi \in \Pi_{prop}^M$ is \emph{$\mathfrak{E}$-stochastic nondominated} if there \emph{does not exist} any policy $\pi' \in \Pi_{prop}^M$ such that $\pi' >_{\mathfrak{E}} \pi$.
\end{definition}

Informally, we say a policy $\pi$ is \emph{$\mathfrak{E}$-preferred} if and only if it is $\mathfrak{E}$-stochastic nondominated in $\Pi_{prop}^M$.

%	We first ask how the user can generate the preference model $\langle \Sigma^\ast, \succeq \rangle$, and then assuming this preference model has been generated, we focus on solving the following planning problem.

We aim to solve the following planning problem:
\begin{problem}
\label{problem:main-problem}
Given a terminating labeled \ac{mdp} $M = \langle S, A:=\bigcup_{s \in S} A_s, \mathbf{P}, s_0, s_\bot, \calAP, L \rangle$, a preference model $\langle \Sigma^\ast, \succeq \rangle$, and a stochastic ordering $\mathfrak{E} \in \{\mathfrak{E}_{st}, \mathfrak{E}_{wk}, \mathfrak{E}_{wk*}\}$, compute a proper policy that is $\mathfrak{E}-$stochastic nondominated.
\end{problem}
% \jf{changed the set to a single policy.}
%
% 		\hrm{
% 		Why informal? A preference model or a \ac{pdfa}? Why we define the problem to compute only a single policy?
% 		%
% 		}




==> sections/synthesis.tex <==
With the computational model \ac{pdfa} representing the partially-ordered temporal goals, we are ready to present a planning algorithm to solve Problem~\ref{problem:main-problem}.
%
The algorithm computes for a given \ac{tlmdp}, a policy that is most-preferred given the user preferences specified by a given \ac{pdfa}. 
%
The first step is to augment the planning state space with the states of the \ac{pdfa}. 
%
With this augmented state space, we can relate the preferences over traces in the \ac{mdp} to a preference over subsets of terminating states in a product \ac{mdp}, defined as follows.
%
\begin{definition}[Product MDP]
\label{def:prod}
Let $M = \langle S, A:=\Sigma_{s \in S}A_s, \mathbf{P}, s_0, s_\bot, \calAP, L \rangle$ and 
$\pdfa = \langle Q, \Sigma, \delta, \init, G:=(\prefnodes, \prefedges)  \rangle$ be respectively the \ac{tlmdp} and the \ac{pdfa}. 
The product of $M$ and $\pdfa$ is a tuple $\calM = (X, A:=\bigcup_{x \in X}A_x, \mathbf{T}, x_0, X_G, \calG := (\augnodes, \augedges))$ in which
\begin{enumerate}
	\item $X =  S \times Q$ is the state space;
	\item $A$ is the action space, where for each $x=(s, q) \in X$, $A_x = A_s$ is the set of available actions at state $x$;
	\item \label{itm:T} $\mathbf{T}: X \times A \rightarrow \dist(X)$ is the transition function such that for each state $(s, q) \in X$, action $a \in A$, and state $(s', q') \in X$;
	\begin{multline*}
		\mathbf{T}((s, q), a, (s', q')) = \\  {
			\begin{cases}
				\mathbf{P}(s, a, s') & \mbox{\text{if} $q' = \delta(q, L(s')),$} \qquad\hfill \\
				0 & \text{otherwise};
			\end{cases}
		}
	\end{multline*}
	\item $x_0 = (s_0, \delta(\init, L(s_0)))$ is the initial state;
	\item $X_G =  \{s_\bot \} \times Q$ is the set of terminating states;
	\item \label{itm:pgraph} $\calG = (\augnodes, \augedges)$ is the preference graph, in which, letting $\augnode_i = \{s_\bot\}\times W_i$ for each $W_i \in \prefnodes$, 
	\begin{itemize}
		\item $\augnodes = \{\augnode_i\mid i=1,\ldots, \abs{\prefnodes}\}$ is the vertex set of the graph, and
		\item $\augedges$ is the edge set of the graph such that $(\augnode_i, \augnode_j)\in \augedges$ if and only if $(W_i, W_j ) \in E$.
	\end{itemize}
\end{enumerate}
\end{definition}

The preference graph of this MDP has been directly lifted from the one defined for the \ac{pdfa}. Given $Y, Y' \in \augnodes$, we use $Y \rightsquigarrow Y'$ to denote 
that $Y'$ is reachable from $Y$ in the preference graph $\calG$. Again, every $Y$ is reachable from itself.
%

\begin{example}
\label{ex:prod_pref_graph}

\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/PDFA.png}
	\caption{
		PDFA for the example in Figure~\ref{fig:gap_garden}. 
		%
		\textbf{Left)} The DFA structure of PDFA.
		%
		\textbf{Right)} The preference graph of PDFA.
		%
	}
	\label{fig:pdfa}
\end{figure}
% \jf{moved this figure   here. please check} 
Figure~\ref{fig:pdfa} shows the \ac{pdfa} constructed for the garden example (Figure~\ref{fig:gap_garden}). We have $\augnode_1 = \{ s_\bot\} \times W_1 = \{(s_\bot, q_2)\}$, $\augnode_2 =\{s_\bot\} \times  W_2=\{(s_\bot, q_4)\}$, $\augnode_3 = \{s_\bot \} \times W_3 = \{(s_\bot, q_1)\}$, and $\augnode_4 = \{s_\bot\} \times W_4 = \{(s_\bot, q_0), (s_\bot, q_3), (s_\bot, q_5)\}$.
\end{example}


Next, we show how to compute a stochastic nondominated policy in the sense of Definition~\ref{def:sto_dominance} through solving a \ac{momdp}. The existence of such a \ac{momdp} is guaranteed by the multi-utility representation theorem \cite[Proposition~1]{ok2002utility}, which states that for every partial order $\langle U, \succeq \rangle$ defined over a finite set $U$, there exists a vector-valued utility function $\mathbf{u}: U \rightarrow \mathbb{R}^n$ such that for any $x, y \in U$, $x \succeq y$ if and only if $\mathbf{u}(x) \geq \mathbf{u}(y)$ where $\geq$ is element-wise\footnote{Specifically, the multi-utility representation theorem \cite[Proposition~1]{ok2002utility} requires the partial order $\succeq$ over the set $U$ to be representable as an intersection of finitely many linear orders. However, \cite{dushnik1941partially,fishburn1985interval} have proved that every partial order over a finite set can be represented as an intersection of finitely many linear orders.}. 

We extend the notions related to stochastic ordering for state subsets of the product MDP $\calM$, constructed  
in Definition~\ref{def:prod}, as follows:
%
%     \begin{definition}
%     \label{def:prod_inc_dec_set}
%     Let $\augnode \in \augnodes$ be a state subset of $\calM$. The upper closure of $\augnode$ is defined by
%     \[
% \{\augnode\}^\uparrow = \bigcup_{\augnode'\in \augnodes, \augnode \rightsquigarrow \augnode'} \{\augnode'\}
% \] and the lower closure of $\augnode$ is defined by
% \[
% \{\augnode\}^\downarrow = \bigcup_{\augnode'\in \augnodes, \augnode' \rightsquigarrow \augnode} \{\augnode'\}.
% \] 
%    Also, $\mathbf{\augnode} \subseteq \augnodes$ is called an \emph{increasing set} if ${\mathbf{\augnode}} = \mathbf{\augnode}^\uparrow$.
%     \end{definition}


\begin{definition}
\label{def:prod_inc_dec_set}
Let $\mathbf{\augnode} \subseteq \augnodes$ be a set of vertices in the preference graph $\mathcal{G}$. The upper closure of $\mathbf{\augnode}$ with respect to $\mathcal{G}$ is defined by 
\[
\mathbf{\augnode}_i^\uparrow = \{\augnode' \mid \exists \augnode \in \mathbf{\augnode}, \augnode\rightsquigarrow \augnode' \}
\] and the lower closure of $\augnode$ is defined by
\[
\mathbf{\augnode}_i^\downarrow = \{\augnode' \mid \exists \augnode \in \mathbf{\augnode}, \augnode' \rightsquigarrow \augnode  \}.
\] 
Also, $ \mathbf{\augnode}  \subseteq \augnodes$ is called an \emph{increasing set} if $ \mathbf{\augnode}   = \mathbf{\augnode}  ^\uparrow$.
\end{definition}
%\aknote{What's $\calG_i$? Not clear. }
%
These sets are used to define a stochastic ordering type as follows:
%
\begin{definition}
Let $\mathfrak{E}_{st}(\augnodes), \mathfrak{E}_{wk}(\augnodes), \mathfrak{E}_{wk*}(\augnodes)$ denote the strong, weak, and weak* orderings, respectively, 
where 
\begin{align*}
\mathfrak{E}_{st}(\augnodes) &= \{\text{ all increasing sets in $2^\augnodes$} \},
\\
\mathfrak{E}_{wk}(\augnodes) &= \{\{\augnode\}^\uparrow \mid \augnode\in \augnodes \} \cup \{\augnodes, \emptyset\},
\\
\mathfrak{E}_{wk*}(\augnodes) &= \{\augnodes\setminus \{\augnode\}^\downarrow \mid \augnode\in \augnodes \} \cup \{\augnodes, \emptyset\},
\end{align*}
\end{definition}   
%
% Note that by construction, the number of subsets
% in $\mathfrak{E}_{wk}(\augnodes)$ minus the empty set and the set $\augnodes$ is exactly the size of $\augnodes$.   
% Let $N = \abs{\augnodes}$. 
%
% \jf{I am ok with indexing the set, but is the notation $\mathcal{I}(\mathfrak{E}(\augnodes))$ necessary? we can always use $ \mathfrak{E}(\augnodes) \setminus \{\augnodes, \emptyset \}$ where this set appears.}
% \hr{Fixed it.}
%
For a stochastic ordering $\mathfrak{E} \in \{\mathfrak{E}_{st}, \mathfrak{E}_{wk}, \mathfrak{E}_{wk*}\}$, 
%let $\mathcal{I}(\mathfrak{E}(\augnodes)) = \mathfrak{E}(\augnodes) \setminus \{\augnodes, \emptyset \}$, $N = \abs{\mathcal{I}(\mathfrak{E}(\augnodes))}$, and 
let the elements of set $\mathfrak{E}(\augnodes) \setminus \{\augnodes, \emptyset \}$ to be indexed arbitrary as $\mathbf{\augnode}_1, \mathbf{\augnode}_2, \cdots, \mathbf{\augnode}_N$.
%
We use this indexed set in the following construction to make a multi-objective MDP. 
%
\begin{definition}[\ac{momdp}]
\label{def:goalMDP}
Given a stochastic ordering $\mathfrak{E} \in \{\mathfrak{E}_{st}, \mathfrak{E}_{wk}, \mathfrak{E}_{wk*}\}$, the multi-objective MDP (MOMDP) associated with the product MDP $\calM = \langle X, A, \mathbf{T}, x_0, X_G, \calG := (\augnodes, \augedges) \rangle$ in Definition~\ref{def:prod} and the stochastic ordering $\mathfrak{E}$, is a tuple $\calP = \langle X, A:=\bigcup_{x \in X} A_x, \mathbf{T}, x_0, X_G, \calZ=\{Z_1, Z_2, \cdots, Z_N \} \rangle$ in which $X$, $A$, $\mathbf{T}$, $x_0$, and $X_G$ are  the same elements in $\calM$ and for each $\mathbf{Y}_i \in \mathfrak{E}(\augnodes) \setminus \{\augnodes, \emptyset \}$, $Z_i = \bigcup_{Y \in \mathbf{Y}_i} Y$.
%
The $i$-th objective in the \ac{momdp} is to maximize the probability for reaching the set $Z_i$.
\end{definition}
%\aknote{Shouldn't there be round-brackets around title of definition. For example: `Definition 17 (MOMDP)'.}
Note that each $Z_i$ is a subset of goal states $X_G$, and that
the intersection of two distinct goal subsets $Z_i$ and $Z_j$ may not be empty.
%

\begin{remark}
We exclude $\augnodes$ and $\emptyset$ from the construction of the multi-objective MDP. This is because we consider only proper policies and under any proper policy, any state in $X_G$ is reached with probability one. As a result, the probability of reaching the objectives $\emptyset$ and $\augnodes$ are always $0$ an $1$, respectively, regardless of the chosen stochastic ordering.
\end{remark}
% Also, consider that because we set $\mathcal{I}(\mathfrak{E}(\augnodes)) = \mathfrak{E}(\augnodes) \setminus \{\augnodes, \emptyset \}$, in the construction of $\mathcal{P}$, we did not make any goal $Z$ for the state subsets $\emptyset$ and $\augnodes$.
% %
% This is because we compute only \emph{proper} policies, which are those policies that with probability $1$ reach the state $X_G$ (recall that because $\prefnodes$ partitions $Q$, $\augnodes$ partitions $X_G$, and thus $\bigcup_{Y \in \augnodes} Y = X_G$), and thus, the probability of reaching the goals $\emptyset$ and $\augnodes$ always respectively be $0$ an $1$, regardless of the chosen stochastic ordering.  

To illustrate the construction of $\mathcal{P}$, we continue with our running example.
%
\begin{example}

Using the running  example in Figure~\ref{fig:pdfa}, for which the preference graph of the product MDP is shown in Example~\ref{ex:prod_pref_graph}, we have
$\{ Y_1\}^\uparrow = \{ Y_1\}$, $\{Y_2 \}^\uparrow = \{Y_1, Y_2 \}$, $\{Y_3\}^\uparrow = \{Y_1, Y_3 \}$, and $\{Y_4\}^\uparrow = \{Y_1, Y_2, Y_3, Y_4 \}$, and as a result,
%    \[
% \mathfrak{E}_{wk}(\augnodes) = \{ \{Y_1\}, \{Y_1, Y_2\}, \{Y_1, Y_3\}, \{Y_1, Y_2, Y_3, Y_4\}, \emptyset \},
% \]
%    and
\[
\mathfrak{E}_{wk}(\augnodes) \setminus \{\augnodes, \emptyset \} = \{ \{Y_1\}, \{Y_1, Y_2\}, \{Y_1, Y_3\} \},
\]
and thus, under weak-stochastic ordering, the MOMDP will have the following objectives
\[
Z_1 = Y_1, Z_2 = Y_1 \cup Y_2, \text{and } Z_3 = Y_1 \cup Y_3.
\]
%
Also, we have $\{Y_1\}^\downarrow = \{Y_1, Y_2, Y_3, Y_4 \}$, $\{Y_2\}^\downarrow = \{Y_2, Y_4 \}$, $\{Y_3\}^\downarrow = \{Y_3, Y_4 \}$, and
% $\{Y_4\}^\downarrow = \{ Y_4\}$, and as a result,
% \[
% 	\mathfrak{E}_{wk*}(\augnodes) = \{ \emptyset, \{Y_1, Y_3\}, \{Y_1, Y_2\}, \{Y_1, Y_2, Y_3\},  \newline \{Y_1, Y_2, Y_3, Y_4\}\},
% 	\]
%  \begin{multline}
	%     \mathfrak{E}_{wk*}(\augnodes) = \{ \emptyset, \{Y_1, Y_3\}, \{Y_1, Y_2\}, \{Y_1, Y_2, Y_3\},  \\ \{Y_1, Y_2, Y_3, Y_4\}\}, \notag
	% \end{multline}
%     and
\[
\mathfrak{E}_{wk*}(\augnodes) \setminus \{\augnodes, \emptyset \}= \{ \{Y_1, Y_3\}, \{Y_1, Y_2\}, \{Y_1, Y_2, Y_3\} \},
\]
and therefore, under weak*-stochastic ordering, the MOMDP will have the following objectives 
\[
Z_1 = Y_1 \cup Y_3, Z_2 = Y_1 \cup Y_2, \text{and } Z_3 = Y_1 \cup Y_2 \cup Y_3.
\]
%
Furthermore, 
%     \[
% \mathfrak{E}_{st}(\augnodes) = \{ \{Y_1\}, \{Y_1, Y_2\}, \{Y_1, Y_3\}, \{Y_1, Y_2, Y_3\}, \{Y_1, Y_2, Y_3, Y_4\}, \emptyset \},
% \]
% \begin{multline}
	%     \mathfrak{E}_{st}(\augnodes) = \{ \{Y_1\}, \{Y_1, Y_2\}, \{Y_1, Y_3\}, \{Y_1, Y_2, Y_3\}, \\ \{Y_1, Y_2, Y_3, Y_4\}, \emptyset \}, \notag
	% \end{multline}
% and, as a result,
\[
\mathfrak{E}_{st}(\augnodes) \setminus \{\augnodes, \emptyset \} = \{ \{Y_1\}, \{Y_1, Y_2\}, \{Y_1, Y_3\}, \{Y_1, Y_2, Y_3\} \},
\]
and hence, under strong-stochastic ordering, the MOMDP will have the following objectives
%    \[
% Z_1 = Y_1, Z_2 = Y_1 \cup Y_2, Z_3 = Y_1 \cup Y_3, \text{and } Z_3 = Y_1 \cup Y_2 \cup Y_3.
% \]
\begin{multline}
	Z_1 = Y_1, Z_2 = Y_1 \cup Y_2, Z_3 = Y_1 \cup Y_3, \text{and } \\ Z_3 = Y_1 \cup Y_2 \cup Y_3. \notag
\end{multline}
%
%
Accordingly, the objectives for each of the stochastic orderings in terms of the temporal goals in Figure~\ref{fig:gap_garden} can
be summarized as Table~\ref{tab:objectives}.

\end{example}



%  \begin{figure}
%   \begin{minipage}[b]{.45\linewidth}
	%     \centering
	%     \includegraphics[width=0.7\linewidth]{figures/preferences.png}
	%     \captionof{figure}{Figure caption}% \caption{Figure caption}
	%   \end{minipage}\hfill
%   \begin{minipage}[b]{.45\linewidth}
	%     \centering
	%     \begin{tabular}{cc}
		%         \hline \hline
		%          \scriptsize Stochastic Ordering & \scriptsize  Objectives \\ 
		%         \hline
		%         \scriptsize Weak & \scriptsize  $\{p_1\}, \{p_1, p_2\}, \{p_1, p_3\}$	 \\
		
		%         \scriptsize Strong & \scriptsize  $\{p_1\}, \{p_1, p_2\}, \{p_1, p_3\}, \{p_1, p_2, p_3\}$	 \\
		
		%          \scriptsize Weak*  & \scriptsize $\{p_1, p_2\}, \{p_1, p_3\}, \{p_1, p_2, p_3\}$  \\
		%         \end{tabular}
	%     \captionof{table}{Table caption}
	%   \end{minipage}
% \end{figure}
\begin{table}[h!]
\setlength{\tabcolsep}{0.2em}
\centering    \captionof{table}{Objectives of different stochastic ordering types for the temporal goals in Figure~\ref{fig:gap_garden}.}

\begin{tabular}{cc}
	\hline \hline
	Stochastic Ordering &   Objectives \\ 
	\hline
	Weak &   $\{p_1\}, \{p_1, p_2\}, \{p_1, p_3\}$	 \\
	
	Strong &  $\{p_1\}, \{p_1, p_2\}, \{p_1, p_3\}, \{p_1, p_2, p_3\}$	 \\
	
	Weak*  &  $\{p_1, p_2\}, \{p_1, p_3\}, \{p_1, p_2, p_3\}$  \\
	\hline
\end{tabular}
\label{tab:objectives}
\end{table}


Given the \ac{momdp} in Definition~\ref{def:goalMDP}, for a given randomized, finite-memory policy $\mu: X^* \rightarrow \dist(A)$, we can compute the value vector of $\mu$ as a $N$-dimensional vector $\mathbf{V}^\mu=[\mathbf{V}_1^\mu, \mathbf{V}_2^\mu, \cdots, \mathbf{V}_N^\mu]$ where for each $i$, $\mathbf{V}_i^\mu$ is the 
probability of reaching states of $Z_i$ by following policy $\mu$, starting from the initial state.

Given a randomized, memoryless policy $\mu: X \rightarrow \dist(A)$, to compute its value vector $\mathbf{V}^\mu$, we first set for each terminating   state $x_g \in X_G$, $\mathbf{V}^\mu(x_g)$ to be the vector such that for each $i \in \{1, \cdots, n \}$, $\mathbf{V}^\mu_i(x_g) = 1$ if $x_g \in Z_i$, and otherwise $\mathbf{V}^\mu_i(x_g) = 0$. Then we compute the values of the non-terminating states $x \in X \setminus X_G$ via the Bellman equation,
%
\begin{equation}
\mathbf{V}^{\mu}(x) = \sum_{a \in A} \left ( \mu(x, a) \sum_{x' \in X} \mathbf{T}(x, a, x') \mathbf{V}^{\mu}(x') \right ).
\end{equation}

\begin{definition}
\label{def:paretoDomPolicy}
Given two proper polices $\mu$ and $\mu'$ for $\calM$, it is said that $\mu$ \emph{Pareto dominates} $\mu'$, 
denoted $\mu > \mu'$, if for each $i \in \{1, \cdots, N\}$, $\mathbf{V}_i^{\mu} \geq \mathbf{V}_i^{\mu'}$, and for at least one $j \in \{1, \cdots, N\}$, $\mathbf{V}_j^{\mu} > \mathbf{V}_j^{\mu'}$.
\end{definition}
%
Intuitively, $\mu$ Pareto dominates $\mu'$ if, compared to $\mu'$, it increases the probability of reaching at least a set $Z_j$ without reducing the probability of reaching other sets $Z_i$'s.

\begin{definition}
\label{def:nonDomPolicy}
A proper policy $\mu$ for the MOMDP   is \emph{Pareto optimal} if for there is no other proper policy $\mu'$ such that $\mu' > \mu$.
\end{definition}
In words, a policy is Pareto optimal if it is not dominated by any policy.
%
The \emph{Pareto front} is the set of all Pareto optimal policies. 
%
%    \hrm{I think we need to keep the definition of "Pareto optimal policy"; otherwise, the "Pareto front" will not be well-defined.}
It is well-known that the set of memoryless policies suffices for achieving the Pareto front ~\cite{chatterjee2006markov}. Thus, we restrict to computing memoryless policies.

With this in mind, we present the following result.
%
\begin{theorem}
\label{thm:pareto-weakstochastic}
Assume the MOMDP $\calP$ in Definition~\ref{def:goalMDP} is constrcuted under a stochastic ordering $\mathfrak{E} \in \{\mathfrak{E}_{st}, \mathfrak{E}_{wk}, \mathfrak{E}_{wk*}\}$ and let $\mu: X \rightarrow \dist(A)$ be a policy for $\calP$.
%
Construct policy $\pi: S^* \rightarrow \dist(A)$ for the \ac{tlmdp} $M$ such that for each $\rho=s_0 s_1 \cdots s_n \in S^*$ it is set
$\pi(\rho) = \mu((s_n, \delta(\iota, \trace(\rho))))$.
%
If $\mu$ is Pareto optimal, then $\pi$ is $\mathfrak{E}$-stochastic nondominated, respecting the preference specified by \ac{pdfa} $\pdfa$.
\end{theorem}
%
\begin{proof}
% It is easy to show by the construction of the product \ac{mdp}, if $\mu$ ensures with probability one,  a termininating state in $X_G$ is reached, then $\pi$ is a proper policy.
%
We first provide a detailed proof of the case where $\mathfrak{E} = \mathfrak{E}_{wk}$, that is, where $\mathcal{P}$ is constructed for weak-stochastic ordering.
%   
We show that if $\mu$ is Pareto optimal then $\pi$ is weak-stochastic nondominated. To facilitate the proof, the following notation is used: Let $\Pr^\mu(\mbox{reach}(H), \calM)$ be the probability of terminating in the set $H \subseteq X$ given the policy $\mu$ for the MOMDP and $\Pr^\pi(\mbox{reach}(P), M)$ be the probability of terminating in the set $P \subseteq S$ given the policy $\pi$ in the original S\ac{tlmdp}. 

% \jf{the following are pointers.}

%  \begin{itemize}
	%       \item First, show that $ \Pr^\mu(\reach{Z_i}, \calM) = \Pr^\pi(\mbox{reach}(F_i^+) , M\}$ where $F_i^+ =\bigcup_{F, F_i \rightsquigarrow F} F $. Using plain words can describe the bijections.
	%      \item  Show that $\Pr^\pi(\mbox{reach}(F_i^+), M) =\Pr^\pi(  \{w\}^\uparrow $) for \emph{any} $w$ such that $\delta(\init, w)\in F_i$.
	%      \item relate the property of Pareto-optimal with the weak stochastic dominancy. 
	% \end{itemize}


First, consider that by the construction of the product MDP, Definition~\ref{def:prod}, preference graphs $\calG$ and $G$ are isomorphic, and thus, each $\augnode_i \in \augnodes$ is mapped to a single $\prefnode_i \in \prefnodes$, and vice versa.
%
%\replaced{Let us}{Let's} 
Define $\prefnode_i^+ = 
\bigcup_{\prefnode: \prefnode_i \rightsquigarrow \prefnode} \prefnode$ for each $\prefnode_i \in \prefnodes$. That is, let $\prefnode_i^+$ include the unions of states in all the nodes that can be reached from $\prefnode_i$ in the preference graph. Note that $\prefnode_i \in \prefnode_i^+$.
%
Given that $\calG$ and $G$ are isomorphic, $\augnode_i \rightsquigarrow \augnode_j$ if and only if $\prefnode_i \rightsquigarrow \prefnode_j$ for all $i, j \in \{1, 2, \cdots, N \}$.
%implying that $\{W_i\}^\uparrow = F_i^+$ for all $i=1,\ldots, N$. 
This combined with that $Z_i = \bigcup_{\augnode \in \{\augnode_i\}^\uparrow} \augnode$ for $i \in \{1, \cdots, N\}$ by Definition~\ref{def:goalMDP}, implies that for each $i$,
%
\begin{equation}
	\label{eq:Zi_Fi}
	\mathbf{V}_i^\mu =  \Pr^\mu(\reach{Z_i}, \calM) = \Pr^\pi(\mbox{reach}(\prefnode_i^+) , M\}.
\end{equation}
%
%\replaced{Let us}{Let's} for each $w \in (2^{AP})^*$, $F_w \in \mathbb{F}$ be the single state subset such that $\delta(\init, w) \in F$.
%
Next, for each $w, w' \in \Sigma^\ast$ such that $\delta(\init, w)=\delta(\init, w')$, it holds that $\{w\}^\uparrow = \{w'\}^\uparrow$.
%
Given this and Lemma~\ref{lem:wUp}, for each $\prefnode_i$ and $w \in \Sigma^\ast$ such that $\delta(\init, w) \in \prefnode_i$, 
%
\begin{equation}
	\label{eq:Fi_W}
	\Pr^\pi(\mbox{reach}(\prefnode_i^+), M) =\Pr^\pi(\{w\}^\uparrow ).
\end{equation}
%
Finally, given that $\mu$ is a Pareto optimal policy, by Definition~\ref{def:paretoDomPolicy} and Definition~\ref{def:nonDomPolicy}, it means there exists no policy $\mu'$ such that 
$\mathbf{V}_i^{\mu'} \geq \mathbf{V}_i^\mu$ for all integers $1 \leq i \leq n$ and 
$\mathbf{V}_j^{\mu'} > \mathbf{V}_j^\mu$ for some integer $1 \leq j \leq n$.
%
This, by (\ref{eq:Zi_Fi}) and (\ref{eq:Fi_W}) and that the set of randomized, memoryless policies suffices for the Pareto front of $\calM$, means there exists no policy $\pi' \in \Pi^M_{prop}$ such that $\Pr^{\pi'}(\{w\}^\uparrow ) \geq \Pr^{\pi}(\{w\}^\uparrow )$ for every $w \in \Sigma^*$ and  $\Pr^{\pi'}(\{w'\}^\uparrow ) > \Pr^{\pi}(\{w'\}^\uparrow )$ for some $w' \in  \Sigma^*$.
%
This, by Definition~\ref{def:weak_dominating_policies} and Definition~\ref{def:sto_dominance}, means that $\pi$ is weak-stochastic nondominated.
%  \newpage 

%\jf{The following are corrected, please double check:} 
Proof for the case where $\mathcal{P}$ is constructed for weak*-stochastic ordering, that is, where $\mathfrak{E} = \mathfrak{E}_{wk*}$, is very similar, except that wherever $\prefnode^+$ is used we use $\overline{\prefnode}^-$, defined as 
$\overline{\prefnode}_i^- =\prefnodes\setminus \left(\bigcup_{\prefnode, \prefnode \rightsquigarrow \prefnode_i} \prefnode\right)$. 
%\added{
	For strong-stochastic ordering, we first construct for all subset $V\subseteq \prefnode$, the set $V^\uparrow = \{\prefnode \mid \exists \prefnode_i \in X, \prefnode_i \rightsquigarrow \prefnode \}$,  then exclude any set $V^\uparrow$ if $ V^\uparrow   \ne V$. Then, for each remaining set $V^\uparrow$, the set of states  contained in $V^\uparrow$ is used to define one reachability objective.
	%} 
%, and wherever $.^\uparrow$ is used we use 
%     $.^\downarrow$.
%
\end{proof}


Given the \ac{momdp}, one can use any existing methods to compute a set of Pareto optimal policies for $\calP$. 
%
For a survey of those methods, see~\cite{roijers2013survey}.
%
Note that computing the set of all Pareto optimal policies is generally infeasible, and thus, one needs to compute only a subset of them or to approximate them.
%

